Physics-based reduced-order modeling of flash-boiling sprays in the context of internal combustion engines

Flash-boiling injection is one of the most effective ways to accomplish improved atomization compared to the high-pressure injection strategy. The tiny droplets formed via flash-boiling lead to fast fuel-air mixing and can subsequently improve combustion performance in engines. Most of the previous studies related to the topic focused on modeling flash-boiling sprays using three-dimensional (3D) computational fluid dynamics (CFD) techniques such as direct numerical simulations (DNS), large-eddy simulations (LES), and Reynolds-averaged Navier-Stokes (RANS) simulations. However, reduced order models can have significant advantages for applications such as the design of experiments, screening novel fuel candidates, and creating digital twins, for instance, because of the lower computational cost. In this study, the previously developed cross-sectionally averaged spray (CAS) model is thus extended for use in simulations of flash-boiling sprays. The present CAS model incorporates several physical submodels in flash-boiling sprays such as those for air entrainment, drag, superheated droplet evaporation, flash-boiling induced breakup, and aerodynamic breakup models. The CAS model is then applied to different fuels to investigate macroscopic spray characteristics such as liquid and vapor penetration lengths under flash-boiling conditions. It is found that the newly developed CAS model captures the trends in global flash-boiling spray characteristics reasonably well for different operating conditions and fuels. Moreover, the CAS model is shown to be faster by up to four orders of magnitude compared with simulations of 3D flash-boiling sprays. The model can be useful for many practical applications as a reduced-order flash-boiling model to perform low-cost computational representations of higher-order complex phenomena.

==> CAS_IJMF/texsrc/references.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for Avijit Saha at 2023-03-21 09:50:33 +0100 


%% Saved with string encoding Unicode (UTF-8) 

@misc{CMT2023,
	author = {CMT},
	note = {{Accessed on 21.03.2023}},
	title = {Virtual injection rate generator, {CMT-Motores T{\'e}r micos, Universitat Polit{\`e}cnica de Val{\`e}ncia}},
	url = {https://www.cmt.upv.es/},
	urldate = {2023},
	year = {2023},
	Bdsk-Url-1 = {https://www.cmt.upv.es/}}

@article{Deshmukh2022b,
	author = {Deshmukh, A. Y. and Davidovic, M. and Grenga, T. and Lakshmanan, R. and Cai, L. and Pitsch, H.},
	date-added = {2023-03-21 08:13:40 +0100},
	date-modified = {2023-03-21 08:17:21 +0100},
	doi = {https://doi.org/10.1016/j.combustflame.2021.111751},
	journal = {Combustion and Flame},
	month = {February},
	pages = {111751},
	title = {A reduced-order model for turbulent reactive sprays in compression ignition engines},
	volume = {236},
	year = {2022}}

@article{Li2017,
	author = {Shiyan Li and Yuyin Zhang and Wenyuan Qi and Bin Xu},
	date-added = {2023-03-21 07:57:47 +0100},
	date-modified = {2023-03-21 07:57:47 +0100},
	doi = {https://doi.org/10.1016/j.expthermflusci.2016.09.004},
	journal = {Experimental Thermal and Fluid Science},
	pages = {{305--312}},
	title = {Quantitative observation on characteristics and breakup of single superheated droplet},
	volume = {80},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.expthermflusci.2016.09.004}}

@conference{Saha2021,
	address = {Edinburgh, Scotland UK},
	author = {Saha, A. and Deshmukh, A. Y. and Grenga, T. and Bode, M. and Grunewald, M. and Kaya, Y. and Kirsch, V. and Reddemann, M. A. and Kneer, R. and Pitsch, H.},
	booktitle = {International Conference on Liquid Atomization and Spray Systems (ICLASS), 30th September - 2nd September},
	date-added = {2023-03-21 07:57:32 +0100},
	date-modified = {2023-03-21 07:57:32 +0100},
	title = {{Numerical Modeling of the Flash Boiling Characteristics of E-Fuels at Low Ambient Pressure}},
	year = {2021}}

@article{Moin1991,
	author = {Moin,P. and Squires,K. and Cabot,W. and Lee,S.},
	date-added = {2023-02-25 09:29:31 +0100},
	date-modified = {2023-02-25 09:29:31 +0100},
	doi = {10.1063/1.858164},
	journal = {Physics of Fluids A: Fluid Dynamics},
	number = {11},
	pages = {2746-2757},
	title = {A dynamic subgrid‐scale model for compressible turbulence and scalar transport},
	volume = {3},
	year = {1991},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.858164}}

@article{Germano1991,
	author = {Germano,Massimo and Piomelli,Ugo and Moin,Parviz and Cabot,William H.},
	date-added = {2023-02-25 09:28:50 +0100},
	date-modified = {2023-02-25 09:28:50 +0100},
	doi = {10.1063/1.857955},
	journal = {Physics of Fluids A: Fluid Dynamics},
	number = {7},
	pages = {1760-1765},
	title = {A dynamic subgrid‐scale eddy viscosity model},
	volume = {3},
	year = {1991},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.857955}}

@article{Saha2023,
	author = {A. Saha and A. Y. Deshmukh and T. Grenga and H. Pitsch},
	date-added = {2023-02-24 16:52:19 +0100},
	date-modified = {2023-02-24 16:54:55 +0100},
 	doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2023.104479},
	journal = {International Journal of Multiphase Flow},
        pages = {104479}, 
	title = {Dimensional analysis of vapor bubble growth considering bubble-bubble interactions in flash boiling microdroplets of highly volatile liquid electrofuels},
        volume = {165},
	year = {2023}}

@article{Rees2020,
	abstract = {Due to current and future environmental and safety issues in space propulsion, typical propellants for upper stage or satellite rocket engines such as the toxic hydrazine are going to be replaced by green propellants like the combination of liquid oxygen and hydrogen or methane. The injection of that kind of cryogenic fluids into the vacuum atmosphere of space leads to a superheated state, which results in a sudden and eruptive atomization due to flash boiling. For a detailed experimental investigation of superheated cryogenic fluids, the new cryogenic test bench M3.3 with a temperature controlled injection system was built at DLR Lampoldshausen. After a first test campaign with high-speed shadowgraphy of flash boiling liquid nitrogen sprays, a laser-based Phase Doppler system was set-up to determine the spatial distributions of droplet velocities and diameters in highly superheated sprays. The spatial distributions revealed a core region with high mean velocities close to the injector orifice. With increasing distance from the injector orifice, the sprays develop a more and more monodisperse pattern. These distributions also showed that atomization due to flash boiling generates finer sprays with growing degrees of superheat. In certain spray regions, two droplet populations varying in their direction of motion, velocity and diameter due to possible recirculation zones were observed. The experimental data of flash boiling liquid nitrogen generated within this study provide a comprehensive data base for the validation of numerical models and further numerical investigations.},
	author = {Rees, Andreas and Araneo, Lucio and Salzmann, Heiko and Lamanna, Grazia and Sender, Joachim and Oschwald, Michael},
	da = {2020/08/03},
	date-added = {2022-12-23 19:41:55 +0100},
	date-modified = {2022-12-23 19:41:55 +0100},
	doi = {10.1007/s00348-020-03020-7},
	id = {Rees2020},
	isbn = {1432-1114},
	journal = {Experiments in Fluids},
	number = {8},
	pages = {182},
	title = {Droplet velocity and diameter distributions in flash boiling liquid nitrogen jets by means of phase Doppler diagnostics},
	ty = {JOUR},
	volume = {61},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1007/s00348-020-03020-7}}

@article{Loureiro2021,
	author = {Loureiro, D. D. and Kronenburg, A. and Reutzsch, J. and Weigand, B. and Vogiatzaki, K.},
	date-added = {2022-12-17 06:51:30 +0100},
	date-modified = {2022-12-17 06:51:30 +0100},
	doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103705},
	journal = {International Journal of Multiphase Flow},
	pages = {{103705}},
	title = {Droplet size distributions in cryogenic flash atomization},
	volume = {142},
	year = {2021},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103705}}

@article{Duronio2022,
	abstract = { Flash-boiling of fuel sprays occurs when a super-heated fuel is discharged into an environment whose pressure is lower than the saturation pressure of the fuel and can dramatically alter spray formation due to complex two-phase flow effects and rapid droplet vaporization. In gasoline direct injection (GDI) engines, typically, it occurs during the injection process when high fuel temperatures make its saturation pressures higher than the in-cylinder one. Flash boiling significantly affects the spray structure and fuel-air mixture formation, with, potentially, if spray collapse is avoided, positive consequences for the engine performance and pollutant emissions. Hence, this paper developed a modelling approach based on the coupling of Eulerian multi-phase and Eulerian-Lagrangian simulations to reproduce flash boiling sprays physics. It allows a comprehensive description of the flash-boiling phenomena that begins within the injector's ducts and continues outside, where a particular mechanism for primary breakup occurs. Experimental data of the Engine Combustion Network (ECN) Spray G injector, covering various operating conditions, were exploited to assess the reliability of the numerical technique adopted. The validation was performed taking into account various parameters such as axial liquid and vapour penetrations, droplet size and images regarding the near-nozzle zone. The numerical model achieves a pretty good level of agreement with the experimental data and, in particular, it is sensitive to the spray behaviour in the different operating conditions. },
	author = {Francesco Duronio and Andrea Di Mascio and Carlo Villante and Michele Anatone and Angelo De Vita},
	date-added = {2022-12-17 06:18:38 +0100},
	date-modified = {2022-12-17 06:20:26 +0100},
	doi = {10.1177/14680874221090732},
	journal = {International Journal of Engine Research},
	number = {0},
	pages = {14680874221090732},
	title = {ECN Spray G: Coupled Eulerian internal nozzle flow and Lagrangian spray simulation in flash boiling conditions},
	volume = {0},
	year = {2022},
	Bdsk-Url-1 = {https://doi.org/10.1177/14680874221090732}}

@article{Guo2019,
	abstract = {In this research, n-hexane flashing jets discharged from two-hole GDI injectors were studied numerically with different superheat levels and inter-hole angles. The mutual interaction between under-expanded flashing jets was discussed in terms of its effect and mechanism. It was found that under certain conditions, the jets deflected towards each other and merged into one jet which moved along the central axis, indicating the occurrence of spray collapse. The spray collapse is ascribed to the pressure drop in the central area between the two jets, which is an effect of the low-pressure cores within individual jets. The pressure drop in the central area is mainly determined by two effects, i.e. the intensity and volume of the low-pressure cores in individual jets, and the formation of the secondary cell which protects the central area from being affected by the ambience. In the transitional stage from non-collapse to fully-collapse, the pressure drop was enhanced with the rise of superheat level or the decrease of inter-hole angle, and the extent of spray collapse increased. Besides, unique shock structures similar to those of under-expanded gaseous twin-jets were formed at high superheat levels, which consist of two primary cells and a secondary cell.},
	author = {Hengjie Guo and Yanfei Li and Hongming Xu and Shijin Shuai and Huiqiang Zhang},
	date-added = {2022-12-15 07:36:17 +0100},
	date-modified = {2022-12-15 07:46:36 +0100},
	doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2019.04.010},
	issn = {0017-9310},
	journal = {International Journal of Heat and Mass Transfer},
	keywords = {Flash boiling, Two-phase flow, Under-expanded, Jet-to-jet interaction, Spray collapse},
	pages = {990-1000},
	title = {Interaction between under-expanded flashing jets: A numerical study},
	volume = {137},
	year = {2019},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0017931019303709},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.ijheatmasstransfer.2019.04.010}}

@article{Guo2019b,
	abstract = {In this paper, n-hexane flashing jets discharged from a single-hole gasoline direct injector (GDI) were studied numerically with the adoption of diffuse Eulerian framework and the homogeneous relaxation model (HRM). The fuel temperature ranged from 30 to 130 $\,^{\circ}$C, and the ambient pressure varied from 20 to 101 kPa. The results showed that considerable vaporization started at the counter bore and a liquid core existed near the nozzle exit. Due to drastic vaporization, the pressure within the liquid core increased so the two-phase flow became under-expanded. Violent expansion then occurred and a low-pressure region was formed, which is believed as the origin of the spray collapse under flashing conditions for multi-hole GDI injectors. At high superheat levels, shock wave structures similar to those in highly under-expanded gaseous jets were identified. However, the transonic position located at some distances from the nozzle rather than at the throttle. Besides, vapor fraction played the dominant role in the onset of expansion, while the expansion was ended by the pressure difference between the two sides of the Mach disk.},
	author = {Hengjie Guo and Yanfei Li and Bo Wang and Huiqiang Zhang and Hongming Xu},
	date-added = {2022-12-15 07:35:28 +0100},
	date-modified = {2022-12-15 07:35:28 +0100},
	doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2018.10.088},
	issn = {0017-9310},
	journal = {International Journal of Heat and Mass Transfer},
	keywords = {Flash boiling, Under-expanded jet, Shock wave, Spray collapse, Low-pressure core},
	pages = {50-59},
	title = {Numerical investigation on flashing jet behaviors of single-hole GDI injector},
	volume = {130},
	year = {2019},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0017931018326164},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.ijheatmasstransfer.2018.10.088}}

@article{Guo2017b,
	abstract = {In this study, the spray characteristics of a five-hole gasoline direct injector were investigated in a constant volume vessel. The absolute ambient pressure ranged from 0.5 to 10.0bar, and the fuel temperatures were 20$\,^{\circ}$C and 80$\,^{\circ}$C. High-speed imaging and phase Doppler measurement technique were utilized to investigate the spray morphology and the droplet dynamics, respectively. Spray collapses were observed in the near field under the elevated ambient pressure (higher than 1.0bar) conditions and in the far field under the flash boiling conditions in both macroscopic and microscopic levels. In addition, under the elevated ambient pressure conditions, the droplets at the inner side of the target jet were larger than those at the outer side, due to the increased probability of droplet coalescence as a result of spray collapse. Whilst, slight increase in droplet diameter in the inner side of the target jet was also found under the flash boiling conditions. Furthermore, the near-field collapse at the elevated ambient pressure conditions was attributed to the jet-air interaction, termed as jet-induced spray collapse; and the far-field collapse under the flash boiling conditions was attributed to the dramatic temperature drop and the resultant vapor condensation, termed as condensation-induced spray collapse.},
	author = {Hengjie Guo and Haichun Ding and Yanfei Li and Xiao Ma and Zhi Wang and Hongming Xu and Jianxin Wang},
	date-added = {2022-12-14 12:27:12 +0100},
	date-modified = {2022-12-14 12:27:12 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2017.02.071},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Gasoline direct injection, Spray collapse, Jet-air interaction, Flash boiling, Condensation},
	pages = {125-134},
	title = {Comparison of spray collapses at elevated ambient pressure and flash boiling conditions using multi-hole gasoline direct injector},
	volume = {199},
	year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236117302247},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2017.02.071}}

@article{Zhou2018,
	abstract = {Flashing spray is of great importance in a variety of engineering fields, which occurs as the pressurized liquid is released into a low-pressure environment below its saturation pressure. The initial stage close to the nozzle exit is furthest from thermodynamic equilibrium and the information of droplets is difficult to obtain by experimental ways due to the high density of droplets. This paper conducts a systematically numerical study on the spray and thermal characteristics of R404A flashing spray with high volatility and low saturation temperature, based on the open source tool OpenFOAM-2.4.0. Key physics involved in the complex process, including droplet flash boiling, evaporation, droplet transport, breakup, heat transfer and interaction between droplet and gas phases are taken into consideration, through Reynolds Averaged Navier Stokes simulations (RANS) with Eulerian Lagrangian framework for the continuous phase and discrete phase respectively. The spray morphology and droplet diameter coincide reasonably with those in the experiment. It presents explosive atomization with large cone angle and quick expansion towards the radial direction near the nozzle exit. Droplet diameter and temperature undergoes a rapid reduction, while velocity accelerates in this region. A warm core with high droplet temperature exists in the spray central region, and droplet velocity is also larger than that at spray periphery. The ambient pressure significantly affects spray profile, penetration distance and velocity. The whole spray profile transforms to the expansion shape as the pressure increases above 0.5 MPa whereby it presents contractive one in low ambient pressure. Higher ambient pressure leads to lower droplet velocity but with longer penetration distance. These numerical results provide further insight into the mechanism of the flashing spray with volatile cryogens.},
	author = {Zhi-Fu Zhou and Guan-Yu Lu and Bin Chen},
	date-added = {2022-12-14 12:26:07 +0100},
	date-modified = {2022-12-14 12:26:07 +0100},
	doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2017.10.095},
	issn = {0017-9310},
	journal = {International Journal of Heat and Mass Transfer},
	keywords = {R404A, Flashing spray, OpenFOAM, Numerical simulation, Spray and thermal characteristics},
	pages = {1312-1321},
	title = {Numerical study on the spray and thermal characteristics of R404A flashing spray using OpenFOAM},
	volume = {117},
	year = {2018},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0017931017330958},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.ijheatmasstransfer.2017.10.095}}

@article{Li2018b,
	abstract = {The main objective of this study is to understand the mechanism of the spray collapse during flash boiling using multi-hole injectors. The spray characteristics of a five-hole gasoline direct injection (GDI) injector were investigated over a range of ambient pressures and fuel temperatures with high-speed imaging and phase Doppler particle measurement techniques. Spray collapses under both flash-boiling and non-flash-boiling (elevated ambient pressure) conditions were observed, but due to different mechanisms. In order to prove that the vapor condensation near the nozzle exit is the primary cause for the collapse under flash boiling conditions, careful analysis to examine the two necessary conditions for vapor condensation in multi-jet flash-boiling sprays was conducted: (1) existence of sub-cooled droplets and (2) existence of saturated vapor. The first condition could be supported by the previous studies and the other condition was numerically and experimentally demonstrated in the present study. It was found that the local static pressure significantly increased at the balance position, where the radial momentums of the droplets and vapor issued from the five holes could be counteracted. The increased static pressure was beyond the local saturation pressure, fulfilling the condition for vapor condensation. Furthermore, the bimodal size distribution under flash boiling conditions and the condensation core inside the spray observed under much reduced ambient pressure also prove the occurrence of vapor condensation at the nozzle exit.},
	author = {Yanfei Li and Hengjie Guo and Shubo Fei and Xiao Ma and Zhou Zhang and Longfei Chen and Liuyang Feng and Zhi Wang},
	date-added = {2022-12-14 12:22:03 +0100},
	date-modified = {2022-12-14 12:22:03 +0100},
	doi = {https://doi.org/10.1016/j.applthermaleng.2018.01.102},
	issn = {1359-4311},
	journal = {Applied Thermal Engineering},
	keywords = {Spray, Collapse, Vapor condensation, Flash boiling, Gasoline direct injection engines},
	pages = {20-28},
	title = {An exploration on collapse mechanism of multi-jet flash-boiling sprays},
	volume = {134},
	year = {2018},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S1359431117331423},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.applthermaleng.2018.01.102}}

@article{Luo2016,
	author = {Luo, Meng and Haidn, Oskar J.},
	date-added = {2022-12-14 12:20:45 +0100},
	date-modified = {2022-12-14 12:21:06 +0100},
	doi = {10.2514/1.B35963},
	journal = {Journal of Propulsion and Power},
	note = {Cited by: 24},
	number = {5},
	pages = {1253 -- 1263},
	publication_stage = {Final},
	source = {Scopus},
	title = {Characterization of Flashing phenomena with cryogenic fluid under vacuum conditions},
	type = {Article},
	volume = {32},
	year = {2016},
	Bdsk-Url-1 = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-84983680236&doi=10.2514%2f1.B35963&partnerID=40&md5=9626ddcb272009587458dd21a556847e},
	Bdsk-Url-2 = {https://doi.org/10.2514/1.B35963}}

@article{Wang2017a,
	abstract = {Knocking combustion research is crucially important because it determines engine durability, fuel consumption, and power density, as well as noise and emission performance. Current spark ignition (SI) engines suffer from both conventional knock and super-knock. Conventional knock limits raising the compression ratio to improve thermal efficiency due to end-gas auto-ignition, while super-knock limits the desired boost to improve the power density of modern gasoline engines due to detonation. Conventional combustion has been widely studied for many years. Although the basic characteristics are clear, the correlation between the knock index and fuel chemistry, pressure oscillations and heat transfer, and auto-ignition front propagation, are still in early stages of understanding. Super-knock combustion in highly boosted spark ignition engines with random pre-ignition events has been intensively studied in the past decade in both academia and industry. These works have mainly focused on the relationship between pre-ignition and super-knock, source analyses of pre-ignition, and the effects of oil/fuel properties on super-knock. The mechanism of super-knock has been recently revealed in rapid compression machines (RCM) under engine-like conditions. It was found that detonation can occur in modern internal combustion engines under high energy density conditions. Thermodynamic conditions and shock waves influence the combustion wave and detonation initiation modes. Three combustion wave modes in the end gas have been visualized as deflagration, sequential auto-ignition and detonation. The most frequently observed detonation initiation mode is shock wave reflection-induced detonation (SWRID). Compared to the effect of shock compression and negative temperature coefficient (NTC) combustion on ignition delay, shock wave reflection is the main cause of near-wall auto-ignition/detonation. Finally, suppression methods for conventional knock and super-knock in SI engines are reviewed, including use of exhaust gas recirculation (EGR), the injection strategy, and the integration of a high tumble - high EGR-Atkinson/Miller cycle. This paper provides deep insights into the processes occurring during knocking combustion in spark ignition engines. Furthermore, knock control strategies and combustion wave modes are summarized, and future research directions, such as turbulence-shock-reaction interaction theory, detonation suppression and utilization, and super-knock solutions, are also discussed.},
	author = {Zhi Wang and Hui Liu and Rolf D Reitz},
	date-added = {2022-12-14 10:16:01 +0100},
	date-modified = {2022-12-14 12:35:58 +0100},
	doi = {https://doi.org/10.1016/j.pecs.2017.03.004},
	issn = {0360-1285},
	journal = {Progress in Energy and Combustion Science},
	keywords = {Knocking combustion, Spark ignition engine, Auto-ignition, Detonation, Super-knock},
	pages = {78-112},
	title = {Knocking combustion in spark-ignition engines},
	volume = {61},
	year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0360128516300764},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.pecs.2017.03.004}}

@article{Aori2016,
	author = {Aori, Gele and Hung, David L.S. and Zhang, Ming and Zhang, Gaoming and Li, Tianyun},
	date-added = {2022-12-14 10:14:31 +0100},
	date-modified = {2022-12-14 10:14:31 +0100},
	doi = {10.1615/AtomizSpr.2015011990},
	journal = {Atomization and Sprays},
	note = {Cited by: 59},
	number = {5},
	pages = {439 -- 462},
	publication_stage = {Final},
	source = {Scopus},
	title = {Effect of nozzle configuration on macroscopic spray characteristics of multi-hole fuel injectors under superheated conditions},
	type = {Article},
	volume = {26},
	year = {2016},
	Bdsk-Url-1 = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-84959274742&doi=10.1615%2fAtomizSpr.2015011990&partnerID=40&md5=85e9d7f18cc32b6496aff51f4afa6429},
	Bdsk-Url-2 = {https://doi.org/10.1615/AtomizSpr.2015011990}}

@article{Araneo2017,
	abstract = {The effects of fuel temperature and chamber pressure on the spray of a multi-hole G-DI injector were analyzed in a quiescent test chamber. The analysis was focused on the behavior of the global spray angles both close and far from the injector. Three pure hydrocarbons (n-hexane, n-heptane, and isooctane), three gasolines of known distillation curve and a commercial 95 RON gasoline from a gas station were utilized. The tests were performed at four chamber pressures (atmospheric, 80kPa, 60kPa and 40kPa) and the fuel temperature was varied from 30$\,^{\circ}$C to 110$\,^{\circ}$C. The results for n-hexane and gasolines were very similar, while n-heptane and isooctane showed a different behavior. The ratio between the fuel saturation pressure at the operating temperature and the air pressure (ps/pa) is confirmed as a fundamental parameter for spray angle data reduction. The near field spray angle data for pure hydrocarbon fuels merge to a unique curve when plotted in function of ps/pa. An approximated method to deduce the gasoline saturation pressure curves starting from the distillation curve is presented. Using the calculated saturation pressures for the reduction of near field spray angle data for the gasolines, a unique curve is obtained, coincident with that of the tested pure hydrocarbons. In alternative, from the results obtained for a fuel of known saturation pressure curve, it is possible to obtain a direct correlation between near field spray angle and saturation pressure. From this relationship, an approximated saturation pressure curve from the experimental angle measurements obtained on the same injector for an unknown fuel can be derived.},
	author = {Lucio Araneo and Roberto Donde'},
	date-added = {2022-12-14 10:11:56 +0100},
	date-modified = {2022-12-14 10:11:56 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2016.11.104},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Flash boiling, Direct injection spark ignition, Spray angle, Gasoline, Distillation curve},
	pages = {500-510},
	title = {Flash boiling in a multihole G-DI injector -- Effects of the fuel distillation curve},
	volume = {191},
	year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236116312133},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2016.11.104}}

@article{Wang2017c,
	abstract = {The characteristics of isooctane spray in the near field and far field were experimentally studied under various flash boiling conditions representing both low load and high load hot engine operation conditions. Closely coupled split injection strategy was also employed to study the influence of flash boiling on the primary breakup of split injections and the interaction between split injections. It was found that flash boiling considerably boosted the spray atomization, especially during the end of injection stage when a large amount of liquid fuel with low speed was observed. The interaction between split injections in liquid phase was significantly weakened under flash boiling condition due to the enhanced atomization but the interaction in gaseous phase was boosted because of the resultant quicker evaporation. The effect of dwell interval on the spray behavior under flash boiling condition was profound, causing significant variation for the delivered fuel mass and spray characteristics.},
	author = {Ziman Wang and Tawfik Badawy and Bo Wang and Yizhou Jiang and Hongming Xu},
	date-added = {2022-12-14 10:10:18 +0100},
	date-modified = {2022-12-14 12:35:53 +0100},
	doi = {https://doi.org/10.1016/j.apenergy.2017.02.009},
	issn = {0306-2619},
	journal = {Applied Energy},
	keywords = {Flash boiling, Primary breakup, Split injection, Spray},
	pages = {199-209},
	title = {Experimental characterization of closely coupled split isooctane sprays under flash boiling conditions},
	volume = {193},
	year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0306261917301241},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.apenergy.2017.02.009}}

@article{Wang2017b,
	abstract = {The effects of deposit on the spray macroscopic characteristics and droplet behaviour under flash boiling condition were investigated through high speed imaging and Phase Doppler Particle Analyzer (PDPA) techniques. Closely coupled split injection strategy was tried to alleviate the negative effect of deposit on spray characteristics. It was found that with single injection strategy, deposit led to smaller cone angle and longer penetration due to poorer atomization and dispersion. Deposit also resulted in larger droplet size by introducing large droplets and lowering the potential of further breakup into small ones. When split injection strategy was employed under non-flash boiling condition, the effects of deposit of on the over-penetration and the resultant high potential of impingement were alleviated, while the negative effect of deposit on droplet size was enhanced. However, when split injection was used under strong flash boiling condition, the negative influence of deposit on the spray over-penetration was significantly alleviated and the negative impact on the droplet size was almost eliminated although reduced potential for large droplets to further break up was still found. The employment of optimal split injection strategy is believed to be important for the alleviation of the adverse effect of deposit on the spray characteristics and the emissions.},
	author = {Ziman Wang and Xiao Ma and Yizhou Jiang and Yanfei Li and Hongming Xu},
	date-added = {2022-12-14 10:09:25 +0100},
	date-modified = {2022-12-14 12:30:29 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2016.11.012},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Deposit, Flash boiling, Split injection, Spray},
	pages = {67-78},
	title = {Influence of deposit on spray behaviour under flash boiling condition with the application of closely coupled split injection strategy},
	volume = {190},
	year = {2017},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236116311073},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2016.11.012}}

@article{Li2018a,
	abstract = {The main objective of this study is to investigate the effect of ambient pressure (Pamb) on the morphology of multi-jet flash boiling sprays and to promote the understanding on the collapse mechanism. With the high-speed imaging technique, the n-hexane spray process in a constant volume vessel was captured under the ambient pressures from 2kPa to 101.3kPa and the fuel temperatures (Tfuel) from 20$\,^{\circ}$C to 120$\,^{\circ}$C. The spray width within the axial distances of 20 nozzle diameters (do) could be increased by increasing Tfuel and/or decreasing Pamb. Beyond 20do, the change in spray width against superheated degree (ΔTSD) was fairly sensitive to Pamb. It decreased with the increase in ΔTSD at Pamb larger than 50kPa, and increased with ΔTSD at Pamb less than 50kPa. Based on the new understanding that the collapse in multi-jet flash-boiling sprays was induced by vapor condensation at the nozzle exit and the resultant local pressure drop (i.e. generation of low-pressure zone), the sensitivity of spray width on Pamb could be well explained as follows: relatively larger Pamb (>50kPa for the used injector) would be conducive to the vapor coagulation and cause stronger vapor condensation (i.e. larger pressure drop) while the vapor dispersion may become dominant at lower Pamb (<50kPa for the used injector), negatively influencing the intensity of vapor condensation.},
	author = {Yanfei Li and Hengjie Guo and Xiao Ma and Yuliang Qi and Zhi Wang and Hongming Xu and Shijin Shuai},
	date-added = {2022-12-14 09:14:53 +0100},
	date-modified = {2022-12-14 12:21:34 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2017.08.082},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Flash boiling, Spray collapse, Gasoline direct injection, Penetration length, Superheated degree, Condensation},
	pages = {38-47},
	title = {Morphology analysis on multi-jet flash-boiling sprays under wide ambient pressures},
	volume = {211},
	year = {2018},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236117310670},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2017.08.082}}

@article{Li2019,
	abstract = {Spray collapse has been widely observed under both flash-boiling and non-flash-boiling conditions when multi-hole gasoline direct injection (GDI) injectors with compact nozzle configurations were used. The main objective of this study is to further understand the collapse mechanisms by using liquids with appreciably different properties (propane, n-hexane and iso-octane). The tests were carried out in a constant volume vessel with ambient pressures ranging from 0.6 bar to 11.0 bar and fuel temperatures from 30 $\,^{\circ}$C to 110 $\,^{\circ}$C. Flashing propane sprays presented a non-collapse feature under elevated-ambient-pressures but flash-boiling conditions. By close-up examination of flashing propane sprays over a wide range of liquid temperatures and ambient pressures, it was found that there should be an ambient pressure threshold between 1.0 and 3.0 bar between the collapsed and the non-collapse sprays for propane. The spray collapse occurred as the ambient pressure is below the threshold. The non-collapse feature for flashing propane sprays under the ambient pressures beyond the threshold was attributed to the prohibition of nucleation and bubble growth under elevated ambient pressures.},
	author = {Yanfei Li and Hengjie Guo and Zhifu Zhou and Zhou Zhang and Xiao Ma and Longfei Chen},
	date-added = {2022-12-14 09:14:21 +0100},
	date-modified = {2022-12-14 09:14:21 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2018.08.160},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Spray, Flash boiling, Gasoline direct injection, Collapse, Nucleation},
	pages = {677-685},
	title = {Spray morphology transformation of propane, n-hexane and iso-octane under flash-boiling conditions},
	volume = {236},
	year = {2019},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236118315308},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2018.08.160}}

@article{Chan2014,
	abstract = {The effect of injection pressure on the structural transformation of flash-boiling sprays of gasoline and ethanol is investigated using a multi-hole injector in an optically accessible, single-cylinder spark-ignition direct-injection (SIDI) engine. The engine was run at 1200 revolutions per minute at wide-open-throttle conditions with no intake air boosting. In fully warmed-up engine environments, high-speed Mie-scattering imaging was performed for two fuel injection timings of 90 and 300 crank angle degrees after top dead centre, corresponding to low and high ambient pressure conditions, respectively. The injection pressure was also varied from 4 to 15MPa. The macroscopic spray structure was quantified using spray tip penetrations, spray spreading angles and spray areas. From the measurements, it is found that fuel sprays injected at the earlier injection timing, when the vapor pressure of the fuel is higher than the ambient pressure, show the convergence of the spray plumes towards the injector axis evidencing the flash-boiling phenomenon. By contrast, fuel injected at the later timing, and hence, higher ambient pressure than the fuel vapor pressure, show typical spray structures with distinct plumes for each nozzle hole. The flash-boiling sprays appear to be influenced by the injection pressure significantly. It is observed that the convergence of spray plumes associated with the flash-boiling is less evident with increasing injection pressure, as higher injection momentum outperforms the plume-to-plume interaction resulting in increased directionality of the spray plumes. It is also found that the enhanced fuel vaporisation due to increased injection pressure is more prevalent in flash-boiling sprays than non-flash-boiling sprays. These findings suggest a great benefit of high pressure injection and flash-boiling sprays in achieving well-mixed charge in SIDI engines. Between gasoline and ethanol, the degree of flash-boiling appears to be different. It is observed that the gasoline sprays undergo flash-boiling and spray collapsing at the low ambient pressure condition while the transitional flash-boiling occurs at the high pressure condition. In comparison, the ethanol sprays experience the transitional flash-boiling at the low pressure condition and no flash-boiling at the high pressure condition. Also, the effect of injection pressure on the spray convergence and fuel vaporisation is more pronounced for the gasoline sprays, all because gasoline fuel has a greater degree of superheating than that of ethanol.},
	author = {Qing N. Chan and Yongming Bao and Sanghoon Kook},
	date-added = {2022-12-14 09:13:07 +0100},
	date-modified = {2022-12-14 09:13:07 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2014.04.015},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Flash-boiling sprays, Injection pressure, Mie-scattering, Gasoline, Ethanol},
	pages = {228-240},
	title = {Effects of injection pressure on the structural transformation of flash-boiling sprays of gasoline and ethanol in a spark-ignition direct-injection (SIDI) engine},
	volume = {130},
	year = {2014},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236114003366},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2014.04.015}}

@article{Aleiferis2010b,
	abstract = {The spray formation and combustion characteristics of gasoline and E85 (85% ethanol, 15% gasoline) have been investigated using a multi-hole injector with asymmetric nozzle-hole arrangement. Experiments were carried out in a quiescent optical chamber using high-speed shadowgraphy (9kHz) to characterise the spray sensitivity to both injector temperature and ambient pressure in the range of 20--120$\,^{\circ}$C and 0.5, 1.0bar. Spray-tip penetrations and `umbrella' spray cone angles were calculated for all conditions. Phase Doppler Anemometry was also used to measure droplet sizes in the core of one of the spray plumes, 25mm below the injector tip. To study the effect of fuel properties on vaporisation and mixture preparation under realistic operating conditions, a separate set of experiments was carried out in a direct-injection spark-ignition optical engine. The engine was run at 1500RPM under cold and fully warmed-up conditions (20$\,^{\circ}$C and 90$\,^{\circ}$C) at part load and full load (0.5 and 1.0bar intake pressure). Floodlit laser Mie-scattering images of the sprays on two orthogonal planes corresponding to the swirl and tumble planes of in-cylinder flow motion were acquired to study the full injection event and post-injection mixing stage. These were used to make comparisons with the static chamber sprays and to quantify the liquid-to-vapour phase evaporation process for both fuels by calculating the projected `footprint' of the sprays at different conditions. Analysis of the macroscopic structure and turbulent primary break-up properties of the sprays was undertaken in light of jet exit conditions described in terms of non-dimensional numbers. The effects on stoichiometric combustion were investigated by imaging the natural flame chemiluminescence through the engine's piston crown (swirl plane) and by post-processing to derive flame growth rates and trajectories of flame motion.},
	author = {P.G. Aleiferis and J. Serras-Pereira and Z. {van Romunde} and J. Caine and M. Wirth},
	date-added = {2022-12-14 09:11:34 +0100},
	date-modified = {2022-12-14 09:11:58 +0100},
	doi = {https://doi.org/10.1016/j.combustflame.2009.12.019},
	issn = {0010-2180},
	journal = {Combustion and Flame},
	keywords = {Spray formation, Combustion, Ethanol, Gasoline, E85, DISI engines},
	number = {4},
	pages = {735-756},
	title = {Mechanisms of spray formation and combustion from a multi-hole injector with E85 and gasoline},
	volume = {157},
	year = {2010},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0010218009003769},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.combustflame.2009.12.019}}

@article{Duronio2021,
	abstract = {Flash boiling is the sudden change from liquid to vapour phase and in IC engines it typically occurs during the injection process with a gasoline direct injection (GDI) setup and when high fuel temperatures result in saturation pressures higher than the in-cylinder ones. The flash boiling, due to the complex evolution of a multi-phase flow and a rapid droplet vaporisation, promotes spray atomisation and affects significantly the spray structure and fuel--air mixture formation, with consequences for the engine performance and pollutant emissions. Hence, a deep knowledge of such phenomenon is required to improve the combustion process and reduce the pollutant production. The breakup mechanism of a superheated spray is quite different from a regular one, because it features the nucleation and growth of bubbles within liquid droplets. In this paper, an innovative flash-boiling breakup model was embedded in a Eulerian--Lagrangian two-phase solver using OpenFOAM library. The model assigns to the droplets a radial velocity component due to the bubble explosion, making it capable of reconstructing the spray expansion. The code was tested using experimental data of the ECN Spray G injector covering various thermodynamic conditions. The numerical model achieves a good level of agreement with the experimental data and, in particular, it is able to reconstruct the spray collapse. Besides, it provides useful information regarding parameters that are intrinsically difficult to measure experimentally.},
	author = {Francesco Duronio and Stefano Ranieri and Alessandro Montanaro and Luigi Allocca and Angelo {De Vita}},
	date-added = {2022-12-14 09:10:14 +0100},
	date-modified = {2022-12-14 09:10:14 +0100},
	doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103817},
	issn = {0301-9322},
	journal = {International Journal of Multiphase Flow},
	keywords = {SprayG, Flash-boiling, OpenFOAM, GDI, CFD, Breakup-modelling},
	pages = {103817},
	title = {ECN Spray G injector: Numerical modelling of flash-boiling breakup and spray collapse},
	volume = {145},
	year = {2021},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0301932221002470},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103817}}

@phdthesis{Robinson2002,
	author = {Robinson, A. J.},
	date-added = {2022-12-11 13:16:54 +0100},
	date-modified = {2022-12-11 13:16:54 +0100},
	title = {{Bubble growth dynamics in boiling}},
	year = {2002}}

@article{Xi2017,
	author = {Xi, Xi and Liu, Hong and Jia, Ming and Xie, Maozhao and Yin, Hongchao},
	date-added = {2022-12-11 13:16:44 +0100},
	date-modified = {2022-12-11 13:16:44 +0100},
	doi = {10.1016/j.ijheatmasstransfer.2016.11.027},
	issn = {00179310},
	journal = {Fuel},
	pages = {{1129--1137}},
	title = {{A new flash boiling model for single droplet}},
	volume = {107},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijheatmasstransfer.2016.11.027}}

@article{Wang2020,
	abstract = {The evaporation and secondary atomization of droplets in cylinder has been confirmed to be one of major factors determining combustion efficiency. Experiments were carried out to elucidate the bubble nucleation and micro-explosion characteristics of superheated jatropha oil (JO) droplet during evaporation process at 873, 973, 1073 K and atmospheric pressure. A single droplet was placed at the intersection of two quartz fiber and introduced rapidly into a high temperature chamber. Several interesting features such as bubble nucleation, bubble growth and coalescence, puffing, vapor jetting, droplet jetting, surface pit, floating raft and micro-explosion were observed. Two different types of micro-explosion, namely global and local micro-explosion were identified. It was also found that chemical reactions occurred during the evaporation process of JO droplet. Bubbles in JO droplet were produced partly by superheating of low boiling point fatty acid and partly by pyrolysis of long-chain fatty acids. There were four modes of bubble nucleation in JO droplet: surface pit nucleation, particle-droplet interface nucleation, fiber-droplet interface nucleation, and floating raft interface nucleation. Surface pit nucleation and floating raft interface nucleation were the main mode. The evaporation residue formed at the end of evaporation, which was caused by the polymerization and aromatization reactions. Most importantly, vapor plume and vapor cloud induced by evaporation have been discovered for the first time. Vapor loud was very similar to the liquid state in the dilute spray region. These were mainly due to the non-isothermal condensation caused by Stefan outflow.},
	author = {Jigang Wang and Xinqi Qiao and Dehao Ju and Chunhua Sun and Tengfei Wang},
	date-added = {2022-12-11 13:16:22 +0100},
	date-modified = {2022-12-11 13:16:22 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2019.116431},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Evaporation, Micro-explosion, Superheat, Jatropha oil, Droplet},
	pages = {116431},
	title = {Bubble nucleation, micro-explosion and residue formation in superheated jatropha oil droplet: The phenomena of vapor plume and vapor cloud},
	url = {https://www.sciencedirect.com/science/article/pii/S0016236119317855},
	volume = {261},
	year = {2020},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236119317855},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2019.116431}}

@article{Wang2019,
	abstract = {Micro-explosion characteristics of soybean oil droplet were investigated using high speed backlight imaging technique at ambient temperature 873 K, 923 K and 973 K. Experimental results indicate that soybean oil droplet underwent transient heating phase, micro-explosion evaporation phase, equilibrium evaporation phase, and residue evaporation phase at all the studied temperatures. The evaporation rate of equilibrium evaporation phase is increased when the temperature increased. However, a decrease for the evaporation rate of residue evaporation phase. Homogeneous and heterogeneous nucleation are observed at all temperatures, homogeneous nucleation lead to strong micro-explosion and heterogeneous nucleation lead to weak micro-explosion. Moreover, micro-explosion strength increased when the ambient increased. It was found that the micro-explosion occurred at the end of droplet evaporation, this is one of the reasons for the poor atomization characteristics of bio-oil in the engine. More importantly, the evaporation induced vapor cloud is observed at 973 K, this is mainly due to the non-isothermal condensation caused by Stefan outflow.},
	author = {Lintao Wang and Jigang Wang and Xinqi Qiao and Dehao Ju and Zhimin Lin},
	date-added = {2022-12-11 13:14:55 +0100},
	date-modified = {2022-12-11 13:14:55 +0100},
	doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2019.04.038},
	issn = {0017-9310},
	journal = {International Journal of Heat and Mass Transfer},
	keywords = {Micro-explosion, Nucleation, Droplet evaporation, Soybean oil, Vapor cloud},
	pages = {736-746},
	title = {Effect of ambient temperature on the micro-explosion characteristics of soybean oil droplet: The phenomenon of evaporation induced vapor cloud},
	url = {https://www.sciencedirect.com/science/article/pii/S001793101930153X},
	volume = {139},
	year = {2019},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S001793101930153X},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.ijheatmasstransfer.2019.04.038}}

@inproceedings{She2010,
	abstract = {Diesel-fuelled homogenous charge compression ignition (HCCI) engines are a new area of focused research as improvements are sought in internal combustion engine technology to reduce energy consumption and air pollution. This paper proposes a new method of utilizing the flash boiling injection effect of high-temperature diesel fuel to improve the fuel-spray evaporation and mixing in HCCI diesel engines. A visual test bench of quasi-stable state fuel injection spray was established, and the influence of high temperature flash boiling injection of diesel fuel on Sauter Mean Diameter (SMD) was tested by laser droplet size analysis. The SMD distributions of diesel engine fuel was measured under different injection pressure and fuel temperatures, and the flash-boiling spray effects on decreasing the fuel droplet diameter, and improving the spray mixture were verified. A Model ZS195, single-cylinder, direct-injection diesel engine was used to test the HCCI combustion efficiency. A section of high-pressure fuel supply pipe with heating and temperature controls was installed following the retrofitted HCCI fuel injection pump. The combustion and exhaust emissions of the HCCI diesel engine were tested for different fuel temperatures, and the effect of high-temperature flash boiling was clearly demonstrated by the test results. In addition, the diesel fuel temperature range to optimize fuel economy and exhaust pollution was identified. Tests were carried out to compare different fuel supply advance angles and injection pressures to ascertain the influence of engine structure and operating parameters on the combustion and emission characteristics. As revealed in the test results, the HCCI combustion diesel engine performance, including fuel consumption and exhaust emissions, were improved by high-temperature flash boiling fuel spray, by increasing the fuel supply advance angle to 32 deg crank angle (CA) before top dead center (BTDC), and increasing the fuel temperature to 160 - 200 deg C.},
	author = {She, Jinping},
	booktitle = {SAE 2010 World Congress \& Exhibition},
	date-added = {2022-12-09 12:27:21 +0100},
	date-modified = {2022-12-09 12:27:21 +0100},
	doi = {https://doi.org/10.4271/2010-01-0341},
	issn = {0148-7191},
	month = {apr},
	publisher = {SAE International},
	title = {Experimental Study on Improvement of Diesel Combustion and Emissions Using Flash Boiling Injection},
	url = {https://doi.org/10.4271/2010-01-0341},
	year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.4271/2010-01-0341}}

@inproceedings{Senda1994,
	abstract = {This paper presents the analysis of atomization and vaporization processes in a flash boiling spray based on experimental results obtained from injection systems in the suction manifold of a gasoline engine. Two kinds of liquid fuel, n-Pentane and n-Hexane, were injected into quiescent atmosphere at room-temperature and low-pressure through a pintle type injector with electronic control. The spray characteristics of both fuels below various atmospheric pressures were investigated in detail by taking photography. Then, in the region of flash boiling, where the back pressure was below the saturated vapor pressure of fuel, the bubble nucleation process due to the flash boiling was modelled by both the measurement results of bubble and the nucleation rate equation using the degree of superheat of the liquid fuel. Further, the fuel vaporization process was assessed by the bubble growth calculation in vapor cavitation phenomena, the fuel evaporation due to boiling from the liquid film surface and the evaporation process from the film surface owing to heat transfer between the ambient gas and the liquid film. Accordingly, the transient change in the bubble diameter and the vapor mass fraction inside the spray are estimated quantitatively for each back pressure. The calculated results, such as the shape of fuel film jet and the fuel droplet diameter in the spray, agree well with the experimental results.},
	author = {Senda, Jiro and Hojyo, Yoshiyuki and Fujimoto, Hajime},
	booktitle = {International Fuels \& Lubricants Meeting \& Exposition},
	date-added = {2022-12-09 12:26:06 +0100},
	date-modified = {2022-12-09 12:26:06 +0100},
	doi = {https://doi.org/10.4271/941925},
	issn = {0148-7191},
	month = {oct},
	publisher = {SAE International},
	title = {Modelling of Atomization Process in Flash Boiling Spray},
	year = {1994},
	Bdsk-Url-1 = {https://doi.org/10.4271/941925}}

@inproceedings{Reitz1987a,
	abstract = {A multi-dimensional model was used to calculate interactions between spray drops and gas motions close to the nozzle in dense high-pressure sprays. The model also accounts for the phenomena of drop breakup, drop collision and coalescence, and the effect of drops, on the gas turbulence. The calculations used a new method to describe atomization (a boundary condition in current spray codes). The method assumes that atomization and drop breakup are indistinguishable processes within the dense spray near the nozzle exit. Accordingly, atomization is prescribed by injecting drops (`blobs') that have a size equal to the nozzle exit diameter. The injected `blobs' breakup due to interaction with the gas as they penetrate, yielding a core region which contains relatively large drops. The computed core length agrees well with available measurements of core length in high-pressure sprays. This core length depends on the operating conditions and it can be comparable to piston-bowl dimensions in internal combustion engine applications. Since the large drops in the core vaporize slowly, these spray structure details are important to the overall spray process. Downstream of the core, drop size in the spray is determined by a competition between drop breakup and drop coalescence, and the computational results agree well with available experimental drop size, drop velocity and spray penetration data.},
	author = {Reitz, Rolf D. and Diwakar, R.},
	booktitle = {SAE International Congress and Exposition},
	date-added = {2022-12-09 12:24:21 +0100},
	date-modified = {2022-12-09 12:24:21 +0100},
	doi = {https://doi.org/10.4271/870598},
	issn = {0148-7191},
	month = {feb},
	publisher = {SAE International},
	title = {Structure of High-Pressure Fuel Sprays},
	year = {1987},
	Bdsk-Url-1 = {https://doi.org/10.4271/870598}}

@article{Ratcliff2016,
	abstract = {Several high octane number oxygenates that could be derived from biomass were blended with gasoline and examined for performance properties and their impact on knock resistance and fine particle emissions in a single cylinder direct-injection spark-ignition engine. The oxygenates included ethanol, isobutanol, anisole, 4-methylanisole, 2-phenylethanol, 2,5-dimethyl furan, and 2,4-xylenol. These were blended into a summertime blendstock for oxygenate blending at levels ranging from 10 to 50 percent by volume. The base gasoline, its blends with p-xylene and p-cymene, and high-octane racing gasoline were tested as controls. Relevant gasoline properties including research octane number (RON), motor octane number, distillation curve, and vapor pressure were measured. Detailed hydrocarbon analysis was used to estimate heat of vaporization and particulate matter index (PMI). Experiments were conducted to measure knock-limited spark advance and particulate matter (PM) emissions. The results show a range of knock resistances that correlate well with RON. Molecules with relatively low boiling point and high vapor pressure had little effect on PM emissions. In contrast, the aromatic oxygenates caused significant increases in PM emissions (factors of 2 to 5) relative to the base gasoline. Thus, any effect of their oxygen atom on increasing local air-fuel ratio was outweighed by their low vapor pressure and high double-bond equivalent values. For most fuels and oxygenate blend components, PMI was a good predictor of PM emissions. However, the high boiling point, low vapor pressure oxygenates 2-phenylethanol and 2,4-xylenol produced lower PM emissions than predicted by PMI. This was likely because they did not fully evaporate and combust, and instead were swept into the lube oil.},
	author = {Ratcliff, Matthew A. and Burton, Jonathan and Sindler, Petr and Christensen, Earl and Fouts, Lisa and Chupka, Gina M. and McCormick, Robert L.},
	date-added = {2022-12-09 12:22:51 +0100},
	date-modified = {2022-12-09 12:22:51 +0100},
	doi = {https://doi.org/10.4271/2016-01-0705},
	issn = {1946-3952},
	journal = {SAE International Journal of Fuels and Lubricants},
	month = {apr},
	number = {1},
	pages = {59--70},
	title = {Knock Resistance and Fine Particle Emissions for Several Biomass-Derived Oxygenates in a Direct-Injection Spark-Ignition Engine},
	url = {https://doi.org/10.4271/2016-01-0705},
	volume = {9},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.4271/2016-01-0705}}

@inproceedings{Price2015,
	abstract = {Flash-boiling of sprays may occur when a superheated liquid is discharged into an ambient environment with lower pressure than its saturation pressure. Such conditions normally exist in direct-injection spark-ignition engines operating at low in-cylinder pressures and/or high fuel temperatures. The addition of novel high volatile additives/fuels may also promote flash-boiling. Fuel flashing plays a significant role in mixture formation by promoting faster breakup and higher fuel evaporation rates compared to non-flashing conditions. Therefore, fundamental understanding of the characteristics of flashing sprays is necessary for the development of more efficient mixture formation. The present computational work focuses on modelling flash-boiling of n-Pentane and iso-Octane sprays using a Lagrangian particle tracking technique. First an evaporation model for superheated droplets is implemented within the computational framework of STAR-CD, along with a full set of temperature dependent fuel properties. Then the computational tool is used to model the injection of flashing sprays through a six-hole asymmetric injector. The computational results are validated against optical experimental data obtained previously with the same injector by high-speed imaging techniques. The effects of ambient pressure (0.5 and 1.0 bar) and fuel temperature (20-180$\,^{\circ}$ C) on the non-flashing and flashing characteristics are examined. Effects of initial droplet size and break-up sub-models are also investigated. The computational methodology is able to reproduce important physical characteristics of flash-boiling sprays like the onset and extent of spray collapse. Based on the current observations, further improvements to the mathematical methodology used for the flash-boiling model are proposed.},
	author = {Price, Christopher and Hamzehloo, Arash and Aleiferis, Pavlos and Richardson, David},
	booktitle = {12th International Conference on Engines \& Vehicles},
	date-added = {2022-12-09 12:22:04 +0100},
	date-modified = {2022-12-09 12:22:10 +0100},
	doi = {https://doi.org/10.4271/2015-24-2463},
	issn = {0148-7191},
	month = {sep},
	publisher = {SAE International},
	title = {Aspects of Numerical Modelling of Flash-Boiling Fuel Sprays},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.4271/2015-24-2463}}

@inproceedings{Patterson1998,
	abstract = {A new spray model has been developed to improve the prediction of diesel engine combustion and emissions using the KIVA-II CFD code. The accuracy of modeling the spray breakup process has been improved by the inclusion of Rayleigh-Taylor accelerative instabilities, which are calculated simultaneously with a Kelvin-Helmholtz wave model. This model improves the prediction of the droplet sizes within a diesel spray and provides a more accurate initial condition for the evaporation, combustion, and emissions models. An improvement to the droplet drag model is also presented. This model accounts for the increased droplet drag due to the change in the droplet's shape, as well as the increase in the frontal area of the droplet. The drag model affects the breakup process locally, producing a more realistic droplet size distribution, and therefore a more accurate calculation of the vaporization process. Through the introduction of this model the prediction of the pressure, heat release, and emissions produced by single and split injections can now be accurately modeled.},
	author = {Patterson, Mark A. and Reitz, Rolf D.},
	booktitle = {International Congress \& Exposition},
	date-added = {2022-12-09 12:21:23 +0100},
	date-modified = {2022-12-09 12:21:23 +0100},
	doi = {https://doi.org/10.4271/980131},
	issn = {0148-7191},
	month = {feb},
	publisher = {SAE International},
	title = {Modeling the Effects of Fuel Spray Characteristics on Diesel Engine Combustion and Emission},
	year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.4271/980131}}

@inproceedings{Kramer2014,
	abstract = {Modern concepts of downsized DI gasoline engines set up high requirements on the injection system to meet the emission targets. The fundamental knowledge and understanding of spray propagation physics are essential for the development of nozzles and injection strategies, due to reduced displacements in combination with the continuing trend of elevated fuel pressures. A detailed analysis of micro- and macroscopic spray parameters was carried out using a multihole solenoid driven DI injector. The measurements were performed in a continuously scavenged pressure chamber with full optical access. Fuel pressure up to 38MPa and backpressures in a range from 0.03 - 0.2 MPa were varied. Optical investigations were done by Shadowgraphy imaging and Phase Doppler Anemometry. The combination of micro- and macroscopic spray results are used to discuss the propagation behaviour of gasoline spray. Against conventional opinions it could be demonstrated that gasoline spray is decelerated at the spray front due to air interactions, even under low gas density conditions. Temporal velocity gradients between the spray front and the following main spray cause droplet overtaking processes. These affect shear zone driven recirculation areas located at the spray front. Reduced penetration values can be achieved by shortening the injection duration. Due to the stopped mass flow and momentum, overtaking processes will stop and penetration stagnates in a constant dimension.},
	author = {Heldmann, Markus and Wensing, Michael and Kr{\"a}mer, Martin and Kull, Eberhard},
	booktitle = {SAE 2014 International Powertrain, Fuels & Lubricants Meeting},
	date-added = {2022-12-09 12:20:25 +0100},
	date-modified = {2022-12-09 12:20:25 +0100},
	doi = {https://doi.org/10.4271/2014-01-2732},
	issn = {0148-7191},
	month = {oct},
	publisher = {SAE International},
	title = {Investigations on Gasoline Spray Propagation Behaviour Characteristic for Multihole Injectors},
	url = {https://doi.org/10.4271/2014-01-2732},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.4271/2014-01-2732}}

@inproceedings{Kawano2004,
	abstract = {Flash-boiling occurs when a fuel is injected to a combustion chamber where the ambient pressure is lower than the saturation pressure of the fuel. It has been known that flashing is a favorable mechanism for atomizing liquid fuels. On the other hand, alternative fuels, such as gaseous fuels and oxygenated fuels, are used to achieve low exhaust emissions in recent years. In general, most of these alternative fuels have high volatility and flash-boiling takes place easily in fuel spray, when they are injected into the combustion chamber of an internal combustion engine under high pressure. In addition, fuel design concept the multicomponent fuel with high and low volatility fuels has been proposed in the previous study in order to control the spray and combustion processes in internal combustion engine. It is found that the multicomponent fuel produce flash-boiling with an increase in the initial fuel temperature. Therefore, it is important to investigate these flash-boiling processes in fuel spray. In the present study, the sub models of flash-boiling spray are constructed. This sub model considers the bubble nucleation, growth and disruption in nozzle orifice and injected fuel droplets. Therefore, the model is implemented into KIVA3V and the spray characteristics of multicomponent fuel with and w/o flashing are numerically investigated. In addition, these numerical results are compared with experimental data which were obtained in the previous study using a constant volume vessel. The flashing spray characteristics from numerical simulation qualitatively shows good agreement with the experimental results. Especially it is confirmed from both the numerical and experimental data that flash-boiling effectively accelerates the atomization and vaporization of fuel droplets. This means that lean homogeneous mixture can be briefly formed by using flash-boiling in combustion chamber.},
	author = {Kawano, Daisuke and Goto, Yuichi and Odaka, Matsuo and Senda, Jiro},
	booktitle = {SAE 2004 World Congress \& Exhibition},
	date-added = {2022-12-09 12:19:33 +0100},
	date-modified = {2022-12-09 12:19:33 +0100},
	doi = {https://doi.org/10.4271/2004-01-0534},
	issn = {0148-7191},
	month = {mar},
	publisher = {SAE International},
	title = {Modeling Atomization and Vaporization Processes of Flash-Boiling Spray},
	year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.4271/2004-01-0534}}

@inproceedings{Adachi1997,
	abstract = {For current passenger vehicles, multi-point injection (MPI) systems are extensively employed for gasoline engines due to ease of control and rapid response. In these systems, the pressure within the intake manifold to which the injectors are installed can fall below the saturated vapor pressure of some hydrocarbon components present in the fuel. Such a condition leads to an atomization process in which flash boiling occurs. In the present work, the atomization process under flash boiling conditions has been characterized both experimentally and theoretically. The experimental investigation has been carried out with a spray test facility consisting of a variable pressure chamber equipped with a pintle type fuel nozzle. Infrared Extinction/Scattering (IRES) is utilized to provide temporal and spatially resolved distribution of the fuel vapor concentration within the spray. Imaging of elastic light scattering from a laser sheet is utilized to characterize the spatial and temporal distribution of the liquid. A theoretical model has been developed for the atomization process taking place for the present spray and compared with the experimental results. The results show that (1) IRES is suitable for application to transient sprays, (2) a correlation exists between vapor concentration and droplet distribution, (3) the amount of vapor increases and becomes uniform over a large volume when the chamber pressure is reduced to cause the flash boiling effect, and (4) the measured vapor mass flux correlate with the modeled mass flux.},
	author = {Adachi, Masayuki and McDonell, Vincent G. and Tanaka, Daisuke and Senda, Jiro and Fujimoto, Hajime},
	booktitle = {International Congress \& Exposition},
	date-added = {2022-12-09 12:18:11 +0100},
	date-modified = {2022-12-09 12:19:16 +0100},
	doi = {https://doi.org/10.4271/970871},
	issn = {0148-7191},
	month = {feb},
	publisher = {SAE International},
	title = {Characterization of Fuel Vapor Concentration Inside a Flash Boiling Spray},
	year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.4271/970871}}

@article{Merola2015,
	abstract = {In this study, experiments were carried out in an optical single-cylinder Direct Injection Spark Ignition engine fuelled with n-butanol and gasoline, alternatively. The engine is equipped with the head of a commercial turbocharged engine with similar geometrical specifications (bore, stroke, compression ratio). The head has four valves and a centrally located spark device with surface charge ignition. A conventional elongated hollow Bowditch piston is used and an optical crown, accommodating fused-silica window, is screwed onto it. The injector is side mounted and features 6 holes oriented to guide the jets towards the piston crown. During the experimental activity, the injection pressure was maintained at 100 bar for all conditions; the injection timing and the number of injections were adjusted to investigate their influence on combustion and emissions. Different optical diagnostics were applied in order to follow the combustion process, from ignition to the completion of flame front propagation: cycle resolved visualization, chemiluminescence and natural emission flame spectroscopy in the UV-Vis range. The optical data was correlated with conventional measurements of thermodynamic analysis and exhaust emissions. The effect of split injection (i.e. two injections per cycle) was found to be relatively negligible for gasoline, while for the alternative fuel significant differences were recorded when switching from single to double injection. This points to a different mixture formation process, mainly related to the evaporative properties of n-butanol.},
	author = {Merola, Simona Silvia and Irimescu, Adrian and Tornatore, Cinzia and Marchitto, Luca and Valentino, Gerardo},
	date-added = {2022-12-09 12:14:45 +0100},
	date-modified = {2022-12-09 12:14:45 +0100},
	doi = {https://doi.org/10.4271/2015-01-0748},
	issn = {1946-3936},
	journal = {SAE International Journal of Engines},
	month = {apr},
	number = {2},
	pages = {474--494},
	title = {Split Injection in a DISI Engine Fuelled with Butanol and Gasoline Analyzed through Integrated Methodologies},
	volume = {8},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.4271/2015-01-0748}}

@article{Sun2021b,
	abstract = {Homogenous, lean combustion has been considered a feasible approach to further improve the performance of the state-of-the-art gasoline direct injection (GDI) engines. However, notable challenges have been seen in properly controlling the lean combustion for satisfactory fuel efficiency and emission performance. To achieve a more homogenous fuel-air mixture for the lean combustion, this manuscript investigated the application of flash boiling atomization in an optical accessible, single cylinder engine operated under lean combustion conditions. Both single injection and split injection schemes were tested and the performance of the engine was evaluated by both traditional and non-intrusive approaches. Imaging methods including micro-LIF-PIV, Mie scattering, and flame chemiluminescence were used to interpret the combustion characteristics inside the engine cylinder. It was found that flash boiling has improved the combustion efficiency, and also PN emission performance if the split injection was used. Spray analysis also indicates that the reason for such phenomena is that fuel-air mixing under flash boiling condition is more complete, thus results in a notably faster flame speed and increased indicative mean effective pressure (IMEP).},
	author = {Zhe Sun and Mingli Cui and Chang Ye and Shangze Yang and Xuesong Li and David Hung and Min Xu},
	date-added = {2022-12-09 12:00:36 +0100},
	date-modified = {2022-12-09 12:05:44 +0100},
	doi = {https://doi.org/10.1016/j.proci.2020.05.037},
	issn = {1540-7489},
	journal = {Proceedings of the Combustion Institute},
	keywords = {Flash boiling atomization, Lean direct injection combustion, Gasoline direct injection engine, Split injection},
	number = {4},
	pages = {5769-5779},
	title = {Split injection flash boiling spray for high efficiency and low emissions in a GDI engine under lean combustion condition},
	volume = {38},
	year = {2021},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S1540748920300857},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.proci.2020.05.037}}

@article{Sun2021a,
	abstract = {Flash boiling atomization is considered a potential solution to multiple issues encountered in fuel atomization for internal combustion engine applications. It has been demonstrated that flash boiling combustion can reduce soot emission under cold-start conditions, while the analysis was still preliminary and limited to engine cold-start conditions. This work investigates the performance of flash boiling combustion in comparison to sub-cooled spray combustions realized with the variation of injection timing. An optical engine facility was used to capture the combustion characteristics with a high-speed color camera, with the temperature of the engine coolant maintained at 60 $\,^{\circ}$C. HSV color model and modified digital CH*/C2* ratio (excess air intensity) to study different flame regions and local combustion richness in the optical engine. The results show that under the conditions tested, flash boiling can improve the efficiency of the engine while reducing the PN emission simultaneously. Furthermore, it was seen that flash boiling combustion could yield a faster flame speed, uniform distribution of flames and less rich mixtures. Finally, color model analysis for transient and averaged flame images is also in good agreement with actual engine performance.},
	author = {Zhe Sun and Mingli Cui and Mohamed Nour and Xuesong Li and David Hung and Min Xu},
	date-added = {2022-12-09 11:59:52 +0100},
	date-modified = {2022-12-09 12:06:04 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2020.119078},
	issn = {0016-2361},
	journal = {Fuel},
	keywords = {Flash boiling combustion, Optical engine, Injection timing, Digital image processing diagnostics},
	pages = {119078},
	title = {Study of flash boiling combustion with different fuel injection timings in an optical engine using digital image processing diagnostics},
	volume = {284},
	year = {2021},
	Bdsk-Url-1 = {https://www.sciencedirect.com/science/article/pii/S0016236120320743},
	Bdsk-Url-2 = {https://doi.org/10.1016/j.fuel.2020.119078}}

@article{Sun2020,
	author = {Sun, Z. and Yang, S. and Nour, M. and Li, X. and Hung, D. and Xu, M.},
	date-added = {2022-12-09 11:56:21 +0100},
	date-modified = {2022-12-09 11:57:50 +0100},
	doi = {https://doi.org/10.1021/acs.energyfuels.0c01942},
	journal = {Energy Fuels},
	pages = {10030--10038},
	title = {Significant Impact of Flash Boiling Spray on In-Cylinder Soot Formation and Oxidation Process},
	volume = {34},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1021/acs.energyfuels.0c01942}}

@article{Shen2016,
	abstract = {An improved extended glare point velocimetry and sizing (EGPVS) is proposed to investigate the droplets sizes of a flash boiling spray. When a spherical droplet with a relative refractive index from 1.16 to 1.41 is illuminated by two opposite laser sheets and a charge-coupled device camera is used to collect the s-polarization light at an observation angle of 90$\,^{\circ}$, the intensities of the reflected lights are much stronger than the other order scattering lights. If the intensity of incident laser is controlled appropriately, two glare points from the reflected lights for the droplet are formed at the focused plane, while the intensities of the other order scattering lights are too weak to form any glare points. Then, the droplet diameter can be derived from the distance between the two glare points. In addition, the focused image is relative small, making it possible to measure dense spray. First, the characteristics of the improved EGPVS are discussed, and a series of standard particles are measured for validating this technique. Then, the technique is applied to investigate the droplets sizes of flash boiling spray. It is found that the minimum measurable diameter of droplets is 7.1 μm, and the relative error is less than 4.7 {\%}. The droplet size distributions of spray are different at different stages. The Sauter mean diameter (SMD) of gasoline spray decreases gradually as the fuel temperature increases, which is different from that of a single-component fuel with a sharp decrease in SMD at the flash boiling stage.},
	author = {Shen, Shiquan and Jia, Ming and Wang, Tianyou and L{\"u}, Qieni and Sun, Kai},
	da = {2016/03/30},
	date-added = {2022-12-09 11:48:01 +0100},
	date-modified = {2022-12-09 11:48:01 +0100},
	doi = {10.1007/s00348-016-2147-3},
	id = {Shen2016},
	isbn = {1432-1114},
	journal = {Experiments in Fluids},
	number = {4},
	pages = {56},
	title = {Measurement of the droplets sizes of a flash boiling spray using an improved extended glare point velocimetry and sizing},
	ty = {JOUR},
	url = {https://doi.org/10.1007/s00348-016-2147-3},
	volume = {57},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1007/s00348-016-2147-3}}

@article{Wang2018,
	author = {Wang, B. and Wang, Z. and Bao, X. and Li, Y. and Jiang, Y. and Xu, H. and Zhang, X.},
	date-added = {2022-12-09 11:41:07 +0100},
	date-modified = {2022-12-09 11:42:50 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2017.10.035},
	journal = {Fuel},
	month = {March},
	pages = {142--152},
	title = {Microscopic investigation of near-field spray characteristics of 2-methylfuran, ethanol and isooctane under flash boiling conditions},
	volume = {215},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2017.10.035}}

@article{Mojtabi2014,
	author = {Mojtabi, M. and Wigley, G. and Helie, J.},
	date-added = {2022-12-09 11:37:47 +0100},
	date-modified = {2022-12-09 11:40:21 +0100},
	doi = {10.1615/AtomizSpr.2014008296},
	journal = {Atomization and Sprays},
	number = {6},
	pages = {467--493},
	title = {The effect of flash boiling on the atomization performance of gasoline direct injection multistream injectors},
	volume = {24},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2014008296}}

@article{Guo2017a,
	author = {Guo, H. and Ma, X. and Li, Y. and Liang, S. and Wang, Z. and Xu, H. and Wang, J.},
	date-added = {2022-12-09 11:32:17 +0100},
	date-modified = {2022-12-14 12:26:41 +0100},
	doi = {http://dx.doi.org/10.1016/j.fuel.2016.11.043},
	journal = {Fuel},
	pages = {79--89},
	title = {Effect of flash boiling on microscopic and macroscopic spray characteristics in optical GDI engine},
	volume = {190},
	year = {2017},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.fuel.2016.11.043}}

@article{Guo2018,
	author = {Guo, H. and Wang, B. and Li, Y. and Xu, H. and Wu, Z.},
	date-added = {2022-12-09 11:29:01 +0100},
	date-modified = {2022-12-09 11:31:12 +0100},
	doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2018.01.042},
	journal = {International Journal of Heat and Mass Transfer},
	pages = {924--932},
	title = {Characterizing external flashing jet from single-hole GDI injector},
	volume = {121},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijheatmasstransfer.2018.01.042}}

@article{Senda2008,
	author = {Senda, J. and Wada, Y. and Kawano, D. and Fujimoto, H.},
	date-added = {2022-12-09 10:02:38 +0100},
	date-modified = {2022-12-09 10:04:42 +0100},
	doi = {10.1243/14680874JER02007},
	journal = {International Journal of Engine Research},
	number = {1},
	pages = {15--27},
	title = {Improvement of combustion and emissions indiesel engines by means of enhanced mixtureformation based on flash boiling of mixed fuel},
	volume = {9},
	year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1243/14680874JER02007}}

@article{Kale2019,
	author = {Kale, Rakesh and Banerjee, R.},
	date-added = {2022-12-09 08:00:42 +0100},
	date-modified = {2022-12-09 08:06:05 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2018.09.142},
	journal = {Fuel},
	pages = {191--201},
	title = {Understanding spray and atomization characteristics of butanol isomers and isooctane under engine like hot injector body conditions},
	volume = {237},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2018.09.142}}

@article{Aleiferis2010a,
	author = {Aleiferis, P. and Serras-Pereira, J. and Augoye, A> and Davies, T. J. and Cracknell, R. F. and Richardson, D.},
	date-added = {2022-12-09 07:23:02 +0100},
	date-modified = {2022-12-14 09:11:55 +0100},
	doi = {10.1016/j.ijheatmasstransfer.2010.06.033},
	journal = {International Journal of Heat and Mass Transfer},
	pages = {4588--4606},
	title = {Effect of fuel temperature on in-nozzle cavitation and spray formation of liquid hydrocarbons and alcohols from a real-size optical injector for direct-injection spark-ignition engines},
	volume = {53},
	year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijheatmasstransfer.2010.06.033}}

@article{Serras2010,
	author = {Serras-Pereira, J. and {van Romunde}, Z. and Aleiferis, P. and Richardson, D. and Wallace, S. and Cracknell, R. F.},
	date-added = {2022-12-09 07:17:43 +0100},
	date-modified = {2022-12-09 07:21:40 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2010.03.030},
	journal = {Fuel},
	pages = {2592--2607},
	title = {Cavitation, primary break-up and flash boiling of gasoline, iso-octane and n-pentane with a real-size optical direct-injection nozzle},
	volume = {89},
	year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2010.03.030}}

@phdthesis{Dietzel2020,
	author = {Dirk Reinhold Dietzel},
	date-added = {2022-12-09 06:09:33 +0100},
	date-modified = {2022-12-09 06:09:33 +0100},
	title = {Modeling and simulation of flash-boiling of cryogenic liquids},
	year = {2020}}

@article{Sher1977,
	author = {Sher, E. and Elata, C.},
	date-added = {2022-12-08 22:04:38 +0100},
	date-modified = {2022-12-08 22:08:55 +0100},
	doi = {https://doi.org/10.1021/i260062a014},
	journal = {Ind. Eng. Chem., Process Des. Dev.},
	number = {2},
	pages = {237--242},
	title = {{Spray Formation from Pressure Cans by Flashing}},
	volume = {16},
	year = {1977},
	Bdsk-Url-1 = {https://doi.org/10.1021/i260062a014}}

@article{Vanderwege1998,
	author = {Vanderwege, Brad A. and Hochgreb, Simone},
	date-added = {2022-12-08 21:44:40 +0100},
	date-modified = {2022-12-08 21:47:40 +0100},
	doi = {https://doi.org/10.1016/S0082-0784(98)80029-5},
	journal = {Symposium (International) on Combustion},
	number = {2},
	pages = {1865--1871},
	title = {The effect of fuel volatility on sprays from high-pressure swirl injectors},
	volume = {27},
	year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0082-0784(98)80029-5}}

@article{Brown1962,
	author = {Brown, R. and York, JL.},
	date-added = {2022-12-08 21:18:52 +0100},
	date-modified = {2022-12-08 21:20:57 +0100},
	journal = {AIChE Journal},
	number = {2},
	pages = {149--53},
	title = {Sprays formed by flashing liquid jets},
	volume = {8},
	year = {1962}}

@article{Badawy2022,
	author = {Badawy, Tawfik and Xu, Hongming and Li, Yanfei},
	date-added = {2022-12-08 21:08:07 +0100},
	date-modified = {2022-12-08 21:10:03 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2021.121820},
	journal = {Fuel},
	pages = {121820},
	title = {Macroscopic spray characteristics of iso-octane, ethanol, gasoline and methanol from a multi-hole injector under flash boiling conditions},
	volume = {307},
	year = {2022},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2021.121820}}

@article{Zeng2012,
	author = {Zeng, Wei and Xu, Min and Zhang, Gaoming and Zhang, Yuyin and Cleary, David J.},
	date-added = {2022-12-08 18:32:03 +0100},
	date-modified = {2022-12-08 18:34:04 +0100},
	doi = {10.1016/j.fuel.2011.08.048},
	journal = {Fuel},
	pages = {287--297},
	title = {Atomization and vaporization for flash-boiling multi-hole sprays with alcohol fuels},
	volume = {95},
	year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2011.08.048}}

@article{Schmitz2002,
	author = {Schmitz, Ingo and Ipp, Wolfgang and Leipertz, Alfred},
	date-added = {2022-12-08 12:59:11 +0100},
	date-modified = {2022-12-09 12:26:36 +0100},
	journal = {SAE Journal of Fuels and Lubricants},
	pages = {1025--1032},
	title = {{Flash Boiling Effects on the Development of Gasoline Direct-Injection Engine Sprays}},
	url = {https://www.jstor.org/stable/44734585},
	volume = {111},
	year = {2002},
	Bdsk-Url-1 = {Stable%20URL:%20https://www.jstor.org/stable/44734585}}

@article{Fujimoto1997,
	author = {Fujimoto, Hajime and Iwami, Yoshiaki and Senda, Jiro},
	date-added = {2022-12-08 12:57:22 +0100},
	date-modified = {2022-12-08 12:58:51 +0100},
	doi = {10.1615/InterJFluidMechRes.v24.i1-3.270},
	journal = {International Journal of Fluid Mechanics Research},
	number = {1--3},
	pages = {273--282},
	title = {{Atomization Characteristics of Liquefied n-Butane Spray with Flash Boiling Phenomena}},
	volume = {24},
	year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.1615/InterJFluidMechRes.v24.i1-3.270}}

@article{Yamazaki1985,
	author = {Yamazaki, Nobuyuki and Miyamoto, Noboru and Murayama, Tadashi},
	date-added = {2022-12-08 12:53:12 +0100},
	date-modified = {2022-12-08 12:56:56 +0100},
	journal = {SAE Transactions},
	pages = {388--395},
	title = {{The Effects of Flash Boiling Fuel Injection on Spray Characteristics, Combustion, and Engine Performance in DI and IDI Diesel Engines}},
	url = {https://www.jstor.org/stable/44467680},
	volume = {94},
	year = {1985},
	Bdsk-Url-1 = {https://www.jstor.org/stable/44467680}}

@article{Sun2021c,
	author = {Sun, Zhe and Xu, Qinglin and Cui, Mingli and Nour, Mohamed and Li, Xuesong and Hung, David L. S.},
	date-added = {2022-12-08 12:04:12 +0100},
	date-modified = {2022-12-09 12:03:09 +0100},
	doi = {https://doi.org/10.1016/j.fuel.2021.121450},
	journal = {Fuel},
	pages = {121450},
	title = {High injection pressure impinging diesel spray characteristics and subsequent soot formation in reacting conditions},
	volume = {304},
	year = {2021},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2021.121450}}

@phdthesis{Zhihao2010,
	author = {Zhao, Zhihao},
	date-added = {2022-12-08 11:09:50 +0100},
	date-modified = {2022-12-08 11:11:51 +0100},
	doi = {https://doi.org/10.37099/mtu.dc.etdr/1318},
	school = {Michigan Technical University},
	title = {High injection pressure impinging diesel spray characteristics and subsequent soot formation in reacting conditions},
	year = {2021},
	Bdsk-Url-1 = {https://doi.org/10.37099/mtu.dc.etdr/1318}}

@article{Xu2013,
	author = {Xu, Min and Zhang, Yuyin and Zeng, Wei and Zhang, Gaoming and Zhang, Ming},
	date-added = {2022-12-08 11:00:51 +0100},
	date-modified = {2022-12-08 11:03:32 +0100},
	doi = {10.4271/2013-01-1614},
	journal = {SAE International Journal of Fuels and Lubricants},
	month = {April},
	number = {1},
	pages = {137--148},
	title = {{Flash Boiling: Easy and Better Way to Generate Ideal Sprays than the High Injection Pressure}},
	volume = {6},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.4271/2013-01-1614}}

@book{Lefebvre1988,
	address = {New York, USA},
	author = {Lefebvre, A. H.},
	date-added = {2022-12-08 10:58:54 +0100},
	date-modified = {2022-12-08 11:00:36 +0100},
	keywords = {Lefebvre, A. H., Atomization and Sprays, Hemisphere Publishing Cooperation, New York, USA, 1988, p. 204},
	publisher = {Hemisphere Publishing Cooperation},
	title = {Atomization and Sprays},
	year = {1988}}

@article{Yang2013,
	author = {Yang, Shenghua and Song, Zhiping and Wang, Tianyou and Yao, Zhuo},
	date-added = {2022-12-08 08:25:05 +0100},
	date-modified = {2022-12-08 08:27:20 +0100},
	doi = {10.1615/AtomizSpr.2013007539},
	journal = {Atomization and Sprays},
	number = {5},
	pages = {379--399},
	title = {An experimental study on phenomenon and mechanism of flash boiling spray from a multi-hole gasoline direct injector},
	volume = {23},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2013007539}}

@article{Reitz2013,
	author = {Reitz, Rolf D.},
	date-added = {2022-12-08 08:23:20 +0100},
	date-modified = {2022-12-08 08:24:31 +0100},
	doi = {https://doi.org/10.1016/j.combustflame.2012.11.002},
	journal = {Combustion and Flame},
	month = {January},
	number = {1},
	pages = {1--8},
	title = {Directions in internal combustion engine research},
	volume = {160},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2012.11.002}}

@book{Zhao2010,
	author = {Zhao, H.},
	date-added = {2022-12-08 08:22:23 +0100},
	date-modified = {2022-12-08 08:23:15 +0100},
	publisher = {Cambridge: Woodhead},
	title = {{Advanced Direct Injection Combustion Engine Technologies and Development: Gasoline and Gas Engines}},
	year = {2010}}

@inbook{Leach2013,
	address = {London},
	author = {Leach, F and Stone, R. and Fennell, D. and Hayden, D. and Richardson, D. and Wicks, N.},
	date-added = {2022-12-08 06:31:34 +0100},
	date-modified = {2022-12-08 06:41:26 +0100},
	doi = {https://doi.org/10.1533/9781782421849.5.193},
	editor = {IMechE},
	month = {November},
	pages = {193--202},
	publisher = {Woodhead Publishing},
	title = {Internal Combustion Engines: Performance, Fuel Economy and Emissions},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1533/9781782421849.5.193}}

@article{Aleiferis2013,
	author = {Aleiferis, Pavlos and {van Romunde}, Z. R.},
	date-added = {2022-12-07 17:26:31 +0100},
	date-modified = {2022-12-07 17:29:58 +0100},
	doi = {http://dx.doi.org/10.1016/j.fuel.2012.07.044},
	journal = {Fuel},
	pages = {143--168},
	title = {An analysis of spray development with iso-octane, n-pentane, gasoline, ethanol and n-butanol from a multi-hole injector under hot fuel conditions},
	volume = {105},
	year = {2013},
	Bdsk-Url-1 = {http://dx.doi.org/10.1016/j.fuel.2012.07.044}}

@article{Price2016,
	author = {Price, Christopher and Hamzehloo, Arash and Aleiferis, Pavlos and Richardson, David},
	date-added = {2022-12-06 06:18:28 +0100},
	date-modified = {2022-12-06 06:20:38 +0100},
	doi = {10.1615/AtomizSpr.2016015807},
	journal = {Atomization and Sprays},
	number = {2},
	pages = {1--43},
	title = {{An Approach to Modeling Flash-Boiling Fuel Sprays for Direct-injection Spark-ignition Engines}},
	volume = {26},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2016015807}}

@article{Gemci2004,
	author = {Gemci, T and Yakut, K and Chigier, N and Ho, T. C.},
	date-added = {2022-12-06 06:14:13 +0100},
	date-modified = {2022-12-06 06:16:41 +0100},
	doi = {doi:10.1016/j.ijmultiphaseflow.2003.12.003},
	journal = {International Journal of Multiphase Flows},
	pages = {395--417},
	title = {Experimental study of flash atomization of binary hydrocarbon liquids},
	volume = {30},
	year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2003.12.003}}

@article{Zeng2001,
	author = {Zeng, Yangbing and Lee, Chia-Fon F.},
	date-added = {2022-12-06 06:09:29 +0100},
	date-modified = {2022-12-14 18:38:05 +0100},
	doi = {http://dx.doi.org/10.1080/00102200108907839},
	journal = {Combustion Science and Technology},
	pages = {45--67},
	title = {{An Atomization Model For Flash Boiling Sprays}},
	volume = {169},
	year = {2001},
	Bdsk-Url-1 = {http://dx.doi.org/10.1080/00102200108907839}}

@article{Yang2017,
	author = {Yang, Shiyou},
	date-added = {2022-11-25 18:37:48 +0100},
	date-modified = {2022-11-25 18:37:48 +0100},
	doi = {10.1615/AtomizSpr.2017020237},
	issn = {10445110},
	journal = {Atomization and Sprays},
	number = {11},
	pages = {{963--997}},
	title = {{Development and validation of a flash boiling model for single-component fuel droplets}},
	volume = {27},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2017020237}}

@article{Price2020,
	author = {Price, C. and Hamzehloo, A. and Aleiferis, P. and Richardson, D.},
	date-added = {2022-11-14 18:55:47 +0100},
	date-modified = {2022-11-14 18:58:24 +0100},
	doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2019.103183},
	journal = {International Journal of Multiphase Flow},
	month = {April},
	pages = {103183},
	title = {Numerical modelling of droplet breakup for flash-boiling fuel spray predictions},
	volume = {125},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2019.103183}}

@article{Saha2022,
	author = {A. Saha and T. Grenga and A. Y. Deshmukh and J. Hinrichs and M. Bode and H. Pitsch},
	date-added = {2022-11-11 13:17:56 +0100},
	date-modified = {2022-11-11 13:17:56 +0100},
	journal = {Fuel},
	pages = {121934},
	title = {Numerical Modeling of Single Droplet Flash Boiling Behavior of E-Fuels Considering Internal and External Vaporization},
	volume = {308},
	year = {2022}}

@article{Zuo2000,
	author = {Zuo, B. and Gomes, A. M. and Rutland, C. J.},
	date-added = {2022-11-11 13:17:33 +0100},
	date-modified = {2022-11-11 13:17:33 +0100},
	doi = {10.1243/1468087001545218},
	journal = {International Journal of Engine Research},
	number = {4},
	pages = {{321--336}},
	title = {{Modelling superheated fuel sprays and vaproization}},
	volume = {1},
	year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1243/1468087001545218}}

@article{Kamoun2010,
	author = {Kamoun, H. and Lamanna, G. and Weigand, B.},
	date-added = {2022-11-11 10:24:58 +0100},
	date-modified = {2022-11-11 10:28:33 +0100},
	journal = {ILASS-Americas 22nd Annual Conference on Liquid Atomization and Spray Systems, Cincinnati, OH},
	month = {May},
	title = {{High-Speed Shadowgraphy Investigations of Superheated Liquid Jet Atomisation}},
	year = {2010}}

@article{Ali2022,
	author = {Ghandilou, A.~J. and Taghavifar, H.},
	date-added = {2022-11-11 10:13:19 +0100},
	date-modified = {2022-11-11 10:32:37 +0100},
	doi = {https://doi.org/10.1080/17597269.2022.2105867},
	journal = {Biofuels},
	number = {9},
	pages = {{1087--1101}},
	title = {New insight into air/spray boundary interaction for diesel and biodiesel fuels under different fuel temperatures},
	volume = {13},
	year = {2022},
	Bdsk-Url-1 = {https://doi.org/10.1080/17597269.2022.2105867}}

@article{Price2018,
	author = {Price, Christopher and Hamzehloo, Arash and Aleiferis, Pavlos and Richardson, David},
	date-added = {2022-11-11 10:12:35 +0100},
	date-modified = {2022-11-11 10:13:13 +0100},
	doi = {10.1016/j.fuel.2018.01.088},
	journal = {Fuel},
	pages = {{518--541}},
	title = {{Numerical modelling of fuel spray formation and collapse from multi-hole injectors under flash-boiling conditions}},
	volume = {221},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2018.01.088}}

@article{Rosin1933,
	author = {Rosin, P and Rammler, E},
	journal = {Journal of the Institute of Fuel},
	pages = {29--36},
	title = {{The Laws Governing the Fineness of powdered coal}},
	volume = {7},
	year = {1933}}

@article{Frossling1938,
	author = {Fr{\"{o}}ssling, Nils},
	journal = {Geophysics},
	pages = {170--216},
	title = {{Uber die verdunstung fallender tropfen}},
	volume = {12},
	year = {1938}}

@article{Nukiyama1939,
	author = {Nukiyama, Shiro and Tanasawa, Yasusi},
	doi = {10.1299/kikai1938.5.136},
	journal = {Transactions of the Japan Society of Mechanical Engineers},
	number = {18},
	pages = {136--143},
	title = {{An Experiment on the Atomization of Liquid. : 4th Report, The Effect of the Properties of Liquid on the Size of Drops.}},
	volume = {5},
	year = {1939},
	Bdsk-Url-1 = {https://doi.org/10.1299/kikai1938.5.136}}

@article{Wilke1950,
	author = {Wilke, C. R.},
	doi = {10.1063/1.1747673},
	journal = {The Journal of Chemical Physics},
	number = {4},
	pages = {517},
	title = {{A viscosity equation for gas mixtures}},
	volume = {18},
	year = {1950},
	Bdsk-Url-1 = {https://doi.org/10.1063/1.1747673}}

@article{Mugele1951,
	author = {Mugele, R. A. and Evans, H. D.},
	doi = {10.1021/ie50498a023},
	journal = {Industrial {\&} Engineering Chemistry},
	number = {6},
	pages = {1317--1324},
	title = {{Droplet Size Distribution in Sprays}},
	volume = {43},
	year = {1951},
	Bdsk-Url-1 = {https://doi.org/10.1021/ie50498a023}}

@article{Ranz1952,
	author = {Ranz, W E and Marshall, W R},
	doi = {10.1016/S0924-7963(01)00032-X},
	isbn = {1111111111},
	issn = {09247963},
	journal = {Chem. Eng. Progr},
	number = {3},
	pages = {141--146; 173--180},
	pmid = {78},
	title = {{Evaporation from drops. Parts I {\&} II.}},
	volume = {48},
	year = {1952},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0924-7963(01)00032-X}}

@article{Lax1954,
	author = {Lax, Peter D.},
	doi = {10.1002/cpa.3160070112},
	journal = {Communications on Pure and Applied Mathematics},
	pages = {159--193},
	title = {{Weak solutions of nonlinear hyperbolic equations and their numerical computation}},
	volume = {7},
	year = {1954},
	Bdsk-Url-1 = {https://doi.org/10.1002/cpa.3160070112}}

@article{Wakuri1959,
	author = {Wakuri, Yutaro and Fujii, Masaru and Amitani, Tatsuo and Tsuneya, Reijiro},
	doi = {10.1299/kikai1938.25.820},
	journal = {Transactions of the Japan Society of Mechanical Engineers},
	number = {156},
	pages = {820--826},
	title = {{Studies on the Penetration of Fuel Spray of Diesel Engine}},
	volume = {25},
	year = {1959},
	Bdsk-Url-1 = {https://doi.org/10.1299/kikai1938.25.820}}

@article{Wakuri1960,
	author = {Wakuri, Yutaro and Fujii, Masaru and Amitani, Tatsuo and Tsuneya, Reijiro},
	doi = {10.1299/jsme1958.3.123},
	journal = {Bulletin of JSME},
	number = {9},
	pages = {123--130},
	title = {{Studies on the Penetration of Fuel Spray in a Diesel Engine}},
	volume = {3},
	year = {1960},
	Bdsk-Url-1 = {https://doi.org/10.1299/jsme1958.3.123}}

@article{Rusanov1961,
	author = {Rusanov, V V},
	journal = {J. Comput. Math. Phys. USSR},
	title = {{Calculation of interaction of non--steady shock waves with obstacles}},
	year = {1961}}

@inproceedings{MacCormack1969,
	address = {Reston, Virigina},
	author = {MacCormack, R.},
	booktitle = {4th Aerodynamic Testing Conference},
	doi = {10.2514/6.1969-354},
	publisher = {American Institute of Aeronautics and Astronautics},
	title = {{The effect of viscosity in hypervelocity impact cratering}},
	year = {1969},
	Bdsk-Url-1 = {https://doi.org/10.2514/6.1969-354}}

@article{Dent1971,
	author = {Dent, J. C.},
	doi = {10.4271/710571},
	journal = {SAE Technical Paper 710571},
	title = {{A basis for the comparison of various experimental methods for studying spray penetration}},
	year = {1971},
	Bdsk-Url-1 = {https://doi.org/10.4271/710571}}

@article{Hay1972,
	author = {Hay, N. and Jones, P. L.},
	doi = {10.4271/720776},
	issn = {26883627},
	journal = {SAE Technical Paper 720776},
	title = {{Comparison of the various correlations for spray penetration}},
	year = {1972},
	Bdsk-Url-1 = {https://doi.org/10.4271/720776}}

@article{Hiroyasu1974,
	author = {Hiroyasu, H. and Kadota, T.},
	doi = {10.4271/740715},
	journal = {SAE Technical Paper 740715},
	title = {{Fuel droplet size distribution in diesel combustion chamber}},
	year = {1974},
	Bdsk-Url-1 = {https://doi.org/10.4271/740715}}

@article{Beam1976,
	author = {Beam, Richard M. and Warming, R. F.},
	doi = {10.1016/0021-9991(76)90110-8},
	issue = {1},
	journal = {Journal of Computational Physics},
	pages = {87--110},
	title = {{An implicit finite-difference algorithm for hyperbolic systems in conservation-law form}},
	volume = {22},
	year = {1976},
	Bdsk-Url-1 = {https://doi.org/10.1016/0021-9991(76)90110-8}}

@article{Hiroyasu1976,
	author = {Hiroyasu, Hiroyuki and Kadota, Toshikazu},
	doi = {10.1299/jsme1958.19.1064},
	issn = {0021-3764},
	journal = {Bull JSME},
	title = {{FUEL DROPLET SIZE DISTRIBUTION IN DIESEL COMBUSTION CHAMBER.}},
	year = {1976},
	Bdsk-Url-1 = {https://doi.org/10.1299/jsme1958.19.1064}}

@article{Hiroyasu1980,
	author = {Hiroyasu, H. and Arai, M.},
	journal = {Trans. JSAE},
	pages = {5--11},
	title = {{Fuel spray penetration and spray angle of diesel engines}},
	volume = {21},
	year = {1980}}

@article{Tamanini1981,
	author = {Tamanini, Francesco},
	doi = {10.1016/S0082-0784(81)80112-9},
	issn = {00820784},
	journal = {Symposium (International) on Combustion},
	title = {{An integral model of turbulent fire plumes}},
	year = {1981},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0082-0784(81)80112-9}}

@article{Jones1982,
	author = {Jones, W. P. and Whitelaw, J. H.},
	doi = {10.1016/0010-2180(82)90112-2},
	issn = {00102180},
	journal = {Combustion and Flame},
	title = {{Calculation methods for reacting turbulent flows: A review}},
	year = {1982},
	Bdsk-Url-1 = {https://doi.org/10.1016/0010-2180(82)90112-2}}

@article{Reitz1986,
	author = {Reitz, Rolf D. and Diwakar, R.},
	doi = {10.4271/860469},
	journal = {SAE Technical Paper 860469},
	pages = {1--7},
	title = {{Effect of Drop Breakup on Fuel Sprays}},
	year = {1986},
	Bdsk-Url-1 = {https://doi.org/10.4271/860469}}

@article{Reitz1987,
	author = {Reitz, Rolf D.},
	journal = {Atomization and Sprays},
	pages = {309--337},
	title = {{Modeling Atomization Processes in High-Pressure Vaporizing Sprays}},
	volume = {3},
	year = {1987}}

@book{Daubert1989,
	author = {Daubert, T. E. and Danner, R P},
	booktitle = {New York : Hemisphere Pub. Corp},
	isbn = {9780891169482},
	publisher = {New York : Hemisphere Pub. Corp},
	title = {{Physical and Thermodynamic Properties of Pure Compounds: Data Compilation}},
	year = {1989}}

@article{Xu1992,
	author = {Xu, Min and Nishida, Keiya and Hiroyasu, Hiroyuki},
	doi = {10.4271/920624},
	journal = {SAE Technical Paper 920624},
	title = {{A practical calculation method for injection pressure and spray penetration in diesel engines}},
	year = {1992},
	Bdsk-Url-1 = {https://doi.org/10.4271/920624}}

@inproceedings{Naber1995,
	address = {San Antonio},
	author = {Naber, J. D. and Siebers, D. L. and Hencken, K. R.},
	booktitle = {Joint Technical Meeting Central and Western States (USA) Sections of the International Combustion Institute},
	pages = {761--766},
	title = {{The Effects of High Ambient Density on Diesel Spray Penetration and Spread}},
	year = {1995}}

@article{Naber1996,
	author = {Naber, Jeffrey and Siebers, Dennis L.},
	doi = {10.4271/960034},
	journal = {SAE Technical Paper 960034},
	title = {{Effects of Gas Density and Vaporization on Penetration and Dispersion of Diesel Sprays}},
	year = {1996},
	Bdsk-Url-1 = {https://doi.org/10.4271/960034}}

@article{Jiang1996,
	author = {Jiang, GS and Shu, CW},
	doi = {10.1006/jcph.1996.0130},
	journal = {Journal of computational physics},
	number = {126},
	pages = {202--228},
	title = {{Efficient implementation of weighted ENO schemes}},
	volume = {228},
	year = {1996},
	Bdsk-Url-1 = {https://doi.org/10.1006/jcph.1996.0130}}

@article{Wan1997a,
	author = {Wan, Y. P. and Peters, N.},
	doi = {10.4271/972866},
	journal = {SAE Technical Paper 972866},
	title = {{Application of the Cross-Sectional Average Method to Calculations of the Dense Spray Region in a Diesel Engine}},
	year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.4271/972866}}

@phdthesis{Wan1997,
	author = {Wan, Y.P.},
	file = {:Users/deshmukh/Library/Application Support/Mendeley Desktop/Downloaded/Wan - 1997 - Numerical Study of Transient Fuel Sprays with Autoignition and Combustion Under Diesel-Engine Relevant Conditions.pdf:pdf},
	school = {RWTH Aachen University},
	title = {{Numerical Study of Transient Fuel Sprays with Autoignition and Combustion Under Diesel-Engine Relevant Conditions}},
	year = {1997}}

@article{Abraham1997,
	author = {Abraham, John},
	doi = {10.4271/970051},
	issn = {26883627},
	journal = {SAE Technical Paper 970051},
	title = {{What is adequate resolution in the numerical computations of transient jets?}},
	year = {1997},
	Bdsk-Url-1 = {https://doi.org/10.4271/970051}}

@article{Siebers1998,
	author = {Siebers, Dennis L.},
	doi = {10.4271/980809},
	issn = {26883627},
	journal = {SAE Technical Paper 980809},
	title = {{Liquid-phase fuel penetration in diesel sprays}},
	year = {1998},
	Bdsk-Url-1 = {https://doi.org/10.4271/980809}}

@article{Sarre1999,
	author = {{von Kuensberg Sarre}, Christopher and Kong, Song-charng and Reitz, Rolf D},
	doi = {10.4271/1999-01-0912},
	journal = {SAE Technical Paper 1999-01-0912},
	number = {724},
	pages = {1--14},
	title = {{Modeling the Effects of Injector Nozzle Geometry on Diesel Sprays}},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.4271/1999-01-0912}}

@article{Kong1999,
	author = {Kong, S. C. and Senecal, P. K. and Reitz, R. D.},
	doi = {10.2516/ogst:1999015},
	journal = {Oil {\&} Gas Science and Technology -- Revue d'IFP Energies nouvelles},
	number = {2},
	pages = {197--204},
	title = {{Developments in Spray Modeling in Diesel and Direct-Injection Gasoline Engines}},
	volume = {54},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.2516/ogst:1999015}}

@article{Siebers1999,
	author = {Siebers, Dennis L.},
	doi = {10.4271/1999-01-0528},
	issn = {26883627},
	journal = {SAE Technical Paper 1999-01-0528},
	title = {{Scaling liquid-phase fuel penetration in diesel sprays based on mixing-limited vaporization}},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.4271/1999-01-0528}}

@article{Miller1999,
	author = {Miller, R. S. and Bellan, J.},
	doi = {10.1017/S0022112098004042},
	journal = {Journal of Fluid Mechanics},
	number = {3},
	pages = {293--338},
	title = {{Direct numerical simulation of a confined three-dimensional gas mixing layer with one evaporating hydrocarbon-droplet-laden stream}},
	volume = {384},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.1017/S0022112098004042}}

@article{Wan1999,
	author = {Wan, Yuepeng and Peters, Norbert},
	doi = {10.1615/AtomizSpr.v9.i2.10},
	journal = {Atomization and Sprays},
	number = {2},
	pages = {111--132},
	title = {{Scaling of Spray Penetration with Evaporation}},
	volume = {9},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.v9.i2.10}}

@article{Beard2000,
	author = {B{\'{e}}ard, P. and Duclos, J. M. and Habchi, C. and Bruneaux, G. and Mokaddem, K. and Baritaud, T.},
	doi = {10.4271/2000-01-1893},
	issn = {26883627},
	journal = {SAE Technical Paper 2000-01-1893},
	title = {{Extension of lagrangian-eulerian spray modeling: Application to high pressure evaporating diesel sprays}},
	year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.4271/2000-01-1893}}

@article{Post2000,
	author = {Post, Scott and Iyer, Venkatraman and Abraham, John},
	doi = {10.1115/1.483268},
	journal = {Journal of Fluids Engineering},
	number = {2},
	pages = {385-395},
	title = {{A study of near-field entrainment in gas jets and sprays under diesel conditions}},
	volume = {122},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.1115/1.483268}}

@article{Sazhin2001,
	author = {Sazhin, S.S. and Feng, G. and Heikal, M.R.},
	doi = {10.1016/S0016-2361(01)00098-9},
	journal = {Fuel},
	number = {15},
	pages = {2171--2180},
	title = {{A model for fuel spray penetration}},
	volume = {80},
	year = {2001},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0016-2361(01)00098-9}}

@article{Han2002,
	author = {Han, Joong-Sub and Lu, Pai-Hsui and Xie, Xing-Bin and Lai, Ming-Chia and Henein, Naeim A.},
	doi = {10.4271/2002-01-2775},
	journal = {SAE Technical Paper 2002-01-2775},
	title = {{Investigation of Diesel Spray Primary Break-up and Development for Different Nozzle Geometries}},
	year = {2002},
	Bdsk-Url-1 = {https://doi.org/10.4271/2002-01-2775}}

@inproceedings{Hasse2002,
	address = {Detroit},
	author = {Hasse, C and Peters, N.},
	booktitle = {11th International Multidimensional Engine Modeling User's Group Meeting},
	publisher = {University of WisconsinMadison, Engine Research Center},
	title = {{Eulerian spray modeling of diesel injection in a highpressure/high temperature chamber}},
	year = {2002}}

@inproceedings{Hasse2003,
	author = {Hasse, C. and Vogel, S. and Peters, N},
	booktitle = {13th International Multidimensional Engine Modeling User's Group Meeting},
	publisher = {Cray Inc.},
	title = {{Modeling of a DaimlerChrysler Truck Engine using an Eulerian Spray Model}},
	year = {2003}}

@article{Desantes2006,
	author = {Desantes, J. M. and Payri, R. and Salvador, F. J. and Gil, A.},
	doi = {10.1016/j.fuel.2005.10.023},
	issue = {1},
	journal = {Fuel},
	pages = {87--110},
	title = {{Development and validation of a theoretical model for diesel spray penetration}},
	volume = {22},
	year = {2006},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2005.10.023}}

@article{Gorokhovski2008,
	author = {Gorokhovski, Mikhael and Herrmann, Marcus},
	doi = {10.1146/annurev.fluid.40.111406.102200},
	journal = {Annual Review of Fluid Mechanics},
	number = {1},
	pages = {343--366},
	title = {{Modeling Primary Atomization}},
	volume = {40},
	year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1146/annurev.fluid.40.111406.102200}}

@article{Pastor2008,
	author = {Pastor, J. V. and {Javier Lopez}, J and Garcia, J and Pastor, J. M.},
	doi = {10.1016/j.fuel.2008.04.017},
	journal = {Fuel},
	number = {13-14},
	pages = {2871--2885},
	title = {{A 1D model for the description of mixing-controlled inert diesel sprays}},
	volume = {87},
	year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2008.04.017}}

@article{Desjardins2008,
	author = {Desjardins, Olivier and Blanquart, Guillaume and Balarac, Guillaume and Pitsch, Heinz},
	doi = {10.1016/j.jcp.2008.03.027},
	issue = {15},
	journal = {Journal of Computational Physics},
	pages = {7125--7159},
	title = {{High order conservative finite difference scheme for variable density low Mach number turbulent flows}},
	volume = {227},
	year = {2008},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.jcp.2008.03.027}}

@article{Desantes2009,
	author = {Desantes, J.M. and Pastor, J.V. and Garc{\'{i}}a-Oliver, J.M. and Pastor, J.M.},
	doi = {10.1016/j.combustflame.2008.10.008},
	journal = {Combustion and Flame},
	number = {1},
	pages = {234--249},
	title = {{A 1D model for the description of mixing-controlled reacting diesel sprays}},
	volume = {156},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2008.10.008}}

@article{Musculus2009,
	author = {Musculus, Mark P.B. and Kattke, Kyle},
	doi = {10.4271/2009-01-1355},
	journal = {SAE Technical Paper 2009-01-1355},
	title = {{Entrainment waves in diesel jets}},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.4271/2009-01-1355}}

@article{Pickett2010,
	author = {Pickett, Lyle M. and Genzale, Caroline L. and Bruneaux, Gilles and Malbec, Louis-Marie and Hermant, Laurent and Christiansen, Caspar and Schramm, Jesper},
	doi = {10.4271/2010-01-2106},
	journal = {SAE International Journal of Engines},
	number = {2},
	pages = {156--181},
	title = {{Comparison of Diesel Spray Combustion in Different High-Temperature, High-Pressure Facilities}},
	volume = {3},
	year = {2010},
	Bdsk-Url-1 = {https://doi.org/10.4271/2010-01-2106}}

@article{Som2011,
	author = {Som, Sibendu and Ramirez, Anita I. and Longman, Douglas E. and Aggarwal, Suresh K.},
	doi = {10.1016/j.fuel.2010.10.048},
	issn = {00162361},
	journal = {Fuel},
	number = {3},
	pages = {1267--1276},
	title = {{Effect of nozzle orifice geometry on spray, combustion, and emission characteristics under diesel engine conditions}},
	volume = {90},
	year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2010.10.048}}

@article{Zhou2011,
	author = {Zhou, Lei and Xie, Mao Zhao and Jia, Ming and Shi, Jun Rui},
	doi = {10.1007/s10409-011-0485-1},
	journal = {Acta Mechanica Sinica},
	pages = {519},
	title = {{Large eddy simulation of fuel injection and mixing process in a diesel engine}},
	volume = {27},
	year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.1007/s10409-011-0485-1}}

@article{Pickett2011,
	author = {Pickett, Lyle M. and Manin, Julien and Genzale, Caroline L. and Siebers, Dennis L. and Musculus, Mark P.B. and Idicheria, Cherian A.},
	doi = {10.4271/2011-01-0686},
	issn = {19463936},
	journal = {SAE International Journal of Engines},
	title = {{Relationship Between Diesel Fuel Spray Vapor Penetration/Dispersion and Local Fuel Mixture Fraction}},
	year = {2011},
	Bdsk-Url-1 = {https://doi.org/10.4271/2011-01-0686}}

@article{Kastengren2012,
	author = {Kastengren, Alan L. and Tilocco, F. Zak and Powell, Christopher F. and Manin, Julien and Pickett, Lyle M. and Payri, Raul and Bazyn, Tim},
	doi = {10.1615/AtomizSpr.2013006309},
	journal = {Atomization and Sprays},
	number = {12},
	pages = {1011--1052},
	title = {{Engine Combustion Network (ECN): Measurements of Nozzle Geometry and Hydraulic Behavior}},
	volume = {22},
	year = {2012},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2013006309}}

@inproceedings{Wehrfritz2012,
	address = {Heidelberg, Germany},
	author = {Wehrfritz, A. and Vuorinen, V. and Kaario, O. and Larmi, M.},
	booktitle = {ICLASS 2012},
	title = {{A High Resolution Study of Non-Reacting Fuel Sprays Using Large-Eddy Simulations}},
	year = {2012}}

@article{Xue2013,
	author = {Xue, Q. and Som, S. and Senecal, P. K. and Pomraning, E.},
	doi = {10.1615/AtomizSpr.2013008320},
	journal = {Atomization and Sprays},
	number = {10},
	pages = {925--955},
	title = {{Large eddy simulation of fuel-spray under non-reacting ic engine conditions}},
	volume = {23},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2013008320}}

@article{Mittal2014,
	author = {Mittal, V. and Kang, S. and Doran, E. and Cook, D. and Pitsch, H.},
	doi = {10.2516/ogst/2013122},
	journal = {Oil {\&} Gas Science and Technology -- Revue d'IFP Energies nouvelles},
	number = {1},
	pages = {29--40},
	title = {{LES of Gas Exchange in IC Engines}},
	volume = {69},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.2516/ogst/2013122}}

@inproceedings{Wang2014,
	author = {Wang, M.M. and Raju, M.M. and Pomraning, E.E. and Kundu, P.P. and Pei, Y.Y. and Som, S.S.},
	booktitle = {Volume 2: Instrumentation, Controls, and Hybrids; Numerical Simulation; Engine Design and Mechanical Development; Keynote Papers},
	doi = {10.1115/ICEF2014-5522},
	publisher = {American Society of Mechanical Engineers},
	title = {{Comparison of Representative Interactive Flamelet and Detailed Chemistry Based Combustion Models for Internal Combustion Engines}},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1115/ICEF2014-5522}}

@incollection{IPCC2014,
	address = {Cambridge},
	author = {{Intergovernmental Panel on Climate Change (IPCC)}},
	booktitle = {Climate Change 2014 Mitigation of Climate Change},
	chapter = {8},
	doi = {10.1017/CBO9781107415416.014},
	editor = {Edenhofer, O. and Pichs-Madruga, R. and Sokona, Y. and Farahani, E. and Kadner, S. and Seyboth, K. and Adler, A. and Baum, I. and Brunner, S. and Eickemeier, P. and Kriemann, B. and Savolainen, J. and Schl{\"{o}}mer, S. and von Stechow, C. and Zwickel, T. and Minx, J.C.},
	pages = {599--670},
	publisher = {Cambridge University Press},
	title = {{Transport}},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1017/CBO9781107415416.014}}

@article{Senecal2014,
	author = {Senecal, P. K. and Pomraning, E. and Richards, K. J. and Som, S.},
	doi = {10.1115/1.4024861},
	journal = {Journal of Energy Resources Technology},
	number = {1},
	pages = {012204},
	title = {{Grid-Convergent Spray Models for Internal Combustion Engine Computational Fluid Dynamics Simulations}},
	volume = {136},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1115/1.4024861}}

@techreport{Bravo2014,
	author = {Bravo, Luis and Kweon, Chol-Bum},
	institution = {Army Research Laboratory},
	title = {{A Review on Liquid Spray Models for Diesel Engine Computational Analysis}},
	year = {2014}}

@article{Bode2015,
	author = {Bode, Mathis and Falkenstein, Tobias and {Le Chenadec}, Vincent and Kang, Seongwon and Pitsch, Heinz and Arima, Toshiyuki and Taniguchi, Hiroyoshi},
	doi = {10.4271/2015-01-0949},
	issn = {01487191},
	journal = {SAE Technical Paper 2015-01-0949},
	title = {{A New Euler/Lagrange Approach for Multiphase Simulations of a Multi-Hole GDI Injector}},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.4271/2015-01-0949}}

@article{Pastor2015,
	author = {Pastor, J. V. and Garc{\'{i}}a-Oliver, J. M. and Pastor, J. M. and Vera-Tudela, W.},
	doi = {10.1615/AtomizSpr.2014010370},
	journal = {Atomization and Sprays},
	number = {6},
	pages = {485--517},
	title = {{One-dimensional diesel spray modeling of multicomponent fuels}},
	volume = {25},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2014010370}}

@article{Skeen2015,
	author = {Skeen, Scott A. and Manin, Julien and Pickett, Lyle M.},
	doi = {10.1016/j.proci.2014.06.040},
	journal = {Proceedings of the Combustion Institute},
	number = {3},
	pages = {3167--3174},
	title = {{Simultaneous formaldehyde PLIF and high-speed schlieren imaging for ignition visualization in high-pressure spray flames}},
	volume = {35},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.proci.2014.06.040}}

@article{Palmer2015,
	author = {Palmer, Johannes and Ramesh, Mogan and Kirsch, Valeri and Reddemann, Manuel and Kneer, Reinhold},
	doi = {10.4271/2015-24-2478},
	issn = {01487191},
	journal = {SAE Technical Paper 2015-24-2478},
	title = {{Spray Analysis of C8H18O Fuel Blends Using High-Speed Schlieren Imaging and Mie Scattering}},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.4271/2015-24-2478}}

@article{Xu2016,
	author = {Xu, Min and Cui, Yi and Deng, Kangyao},
	doi = {10.1016/j.joei.2015.01.002},
	journal = {Journal of the Energy Institute},
	number = {1},
	pages = {138--149},
	title = {{One-dimensional model on liquid-phase fuel penetration in diesel sprays}},
	volume = {89},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.joei.2015.01.002}}

@book{USEIA2016,
	author = {{U. S. Energy Information Administration}},
	booktitle = {International Energy Outlook 2016},
	pages = {5},
	title = {{International Energy Outlook 2016}},
	year = {2016}}

@article{Wei2017,
	author = {Wei, Haiqiao and Chen, Xi and Zhao, Wanhui and Zhou, Lei and Chen, Rui},
	doi = {10.1177/0954407016687478},
	journal = {Proceedings of the Institution of Mechanical Engineers, Part D: Journal of Automobile Engineering},
	number = {14},
	pages = {1877--1888},
	title = {{Effects of the turbulence model and the spray model on predictions of the n-heptane jet fuel--air mixing and the ignition characteristics with a reduced chemistry mechanism}},
	volume = {231},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1177/0954407016687478}}

@manual{Richards2017,
	address = {Madison, WI},
	author = {Richards, K.J. and Senecal, P.K. and Pomraning, E.},
	organization = {Convergent Science Inc},
	title = {{CONVERGE (v2.4)}},
	year = {2017}}

@article{Payri2017,
	author = {Payri, R. and Salvador, F. J. and {De la Morena}, J. and Pagano, V.},
	doi = {10.1016/j.applthermaleng.2017.06.102},
	issn = {13594311},
	journal = {Applied Thermal Engineering},
	keywords = {1D model,Diesel,Ignition delay,Nozzle geometry},
	title = {{Using a one-dimensional spray model to improve liquid length and ignition delay estimations for diesel flames}},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.applthermaleng.2017.06.102}}

@article{Jochim2017,
	author = {Jochim, Bernhard and Korkmaz, Metin and Pitsch, Heinz},
	doi = {10.1016/j.combustflame.2016.08.003},
	issn = {15562921},
	journal = {Combustion and Flame},
	keywords = {Diesel engine combustion,Low-temperature combustion,Multi-zone modeling,Representative interactive flamelet model,Scalar dissipation rate},
	title = {{Scalar dissipation rate based multi-zone model for early-injected and conventional diesel engine combustion}},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2016.08.003}}

@article{Davidovic2017,
	author = {Davidovic, Marco and Falkenstein, Tobias and Bode, Mathis and Cai, Liming and Kang, Seongwon and Hinrichs, J{\"{o}}rn and Pitsch, Heinz},
	doi = {10.2516/ogst/2017019},
	issn = {19538189},
	journal = {Oil and Gas Science and Technology - Rev. IFP Energies nouvelles},
	number = {5},
	title = {{LES of n -Dodecane Spray Combustion Using a Multiple Representative Interactive Flamelets Model}},
	volume = {72},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.2516/ogst/2017019}}

@article{Sen2017,
	author = {Sen, Burak and Ercan, Tolga and Tatari, Omer},
	doi = {10.1016/j.jclepro.2016.09.046},
	issn = {09596526},
	journal = {Journal of Cleaner Production},
	keywords = {Air pollution externalities,Alternative fuel technology,Battery-electric trucks,Heavy-duty trucks,Life-cycle assessment,Regional electricity generation analysis},
	title = {{Does a battery-electric truck make a difference? -- Life cycle emissions, costs, and externality analysis of alternative fuel-powered Class 8 heavy-duty trucks in the United States}},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.jclepro.2016.09.046}}

@article{Kahila2018,
	author = {Kahila, Heikki and Wehrfritz, Armin and Kaario, Ossi and {Ghaderi Masouleh}, Mahdi and Maes, Noud and Somers, Bart and Vuorinen, Ville},
	doi = {10.1016/j.combustflame.2018.01.004},
	journal = {Combustion and Flame},
	pages = {142--159},
	title = {{Large-eddy simulation on the influence of injection pressure in reacting Spray A}},
	volume = {191},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2018.01.004}}

@misc{EuropeanCommission2018,
	author = {{EU Comission}},
	title = {{Communication from The Commission to The European Parliament, The European Council, The Council, The European Economic And Social Committee, The Committee of The Regions and The European Investment Bank A Clean Planet for all A European strategic long-term vision for a prosperous, modern, competitive and climate neutral economy}},
	url = {https://eur-lex.europa.eu/legal-content/EN/TXT/PDF/?uri=CELEX:52018DC0773&from=EN},
	year = {2018},
	Bdsk-Url-1 = {https://eur-lex.europa.eu/legal-content/EN/TXT/PDF/?uri=CELEX:52018DC0773&from=EN}}

@article{Rupp2018,
	author = {Rupp, Matthias and Schulze, Sven and Kuperjans, Isabel},
	doi = {10.3390/wevj9020033},
	journal = {World Electric Vehicle Journal},
	number = {2},
	pages = {33},
	title = {{Comparative Life Cycle Analysis of Conventional and Hybrid Heavy-Duty Trucks}},
	volume = {9},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.3390/wevj9020033}}

@article{Mareev2018,
	author = {Mareev, Ivan and Becker, Jan and Sauer, Dirk Uwe},
	doi = {10.3390/en11010055},
	issn = {19961073},
	journal = {Energies},
	keywords = {Battery electric truck,Energy consumption,Life cycle costs,Long-haul transportation,Vehicle simulation},
	title = {{Battery dimensioning and life cycle costs analysis for a heavy-duty truck considering the requirements of long-haul transportation}},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.3390/en11010055}}

@article{Feng2019,
	author = {Feng, Zehao and Tang, Chenglong and Yin, Yue and Zhang, Peng and Huang, Zuohua},
	doi = {10.1016/j.ijheatmasstransfer.2018.12.147},
	journal = {International Journal of Heat and Mass Transfer},
	pages = {745--755},
	title = {{Time-resolved droplet size and velocity distributions in a dilute region of a high-pressure pulsed diesel spray}},
	volume = {133},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijheatmasstransfer.2018.12.147}}

@article{Senecal2019,
	author = {Senecal, P. K. and Leach, Felix},
	doi = {10.1016/j.rineng.2019.100060},
	journal = {Results in Engineering},
	title = {{Diversity in transportation: Why a mix of propulsion technologies is the way forward for the future fleet}},
	volume = {4},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.rineng.2019.100060}}

@article{Rupp2019,
	author = {Rupp, Matthias and Handschuh, Nils and Rieke, Christian and Kuperjans, Isabel},
	doi = {10.1016/j.apenergy.2019.01.059},
	journal = {Applied Energy},
	pages = {618--634},
	title = {{Contribution of country-specific electricity mix and charging time to environmental impact of battery electric vehicles: A case study of electric buses in Germany}},
	volume = {237},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.apenergy.2019.01.059}}

@misc{VIR2020,
	author = {Payri, R. and Salvador, F.J. and Gimeno, J. and Bracho, G.},
	note = {{Accessed on 12.10.2020}},
	title = {{Virtual Injection Rate Generator}},
	url = {https://www.cmt.upv.es/ECN03.aspx},
	urldate = {2020},
	year = {2020},
	Bdsk-Url-1 = {https://www.cmt.upv.es/ECN03.aspx}}

@misc{FSC2020,
	author = {FSC},
	note = {{Accessed on 12.10.2020}},
	title = {{The Fuel Science Center (FSC)}},
	url = {http://www.fuelcenter.rwth-aachen.de/},
	urldate = {2020},
	year = {2020},
	Bdsk-Url-1 = {http://www.fuelcenter.rwth-aachen.de/}}

@misc{ECN2020,
	author = {ECN},
	note = {{Accessed on 12.10.2020}},
	title = {{Engine Combustion Network (ECN)}},
	url = {https://ecn.sandia.gov/},
	urldate = {2020},
	year = {2020},
	Bdsk-Url-1 = {https://ecn.sandia.gov/}}

@misc{FES2020,
	author = {{Future Energy Systems}},
	note = {{Accessed 12.10.2020}},
	title = {{Future Energy Systems}},
	url = {https://www.futureenergysystems.ca/research/sustainability/biomass},
	urldate = {2020},
	year = {2020},
	Bdsk-Url-1 = {https://www.futureenergysystems.ca/research/sustainability/biomass}}

@article{Helmers2020,
	author = {Helmers, Eckard and Dietz, Johannes and Weiss, Martin},
	doi = {10.3390/su12031241},
	journal = {Sustainability (Switzerland)},
	number = {3},
	pages = {1241},
	title = {{Sensitivity analysis in the life-cycle assessment of electric vs. combustion engine cars under approximate real-world conditions}},
	volume = {12},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.3390/su12031241}}

@misc{COOPTIMA2020,
	author = {{Co-Optima}},
	note = {{Accessed on 12.10.2020}},
	title = {{Co-Optimization of Fuels and Engines}},
	url = {https://www.energy.gov/eere/bioenergy/co-optimization-fuels-engines},
	year = {2020},
	Bdsk-Url-1 = {https://www.energy.gov/eere/bioenergy/co-optimization-fuels-engines}}

@article{Agarwal2019,
	author = {Agarwal, Arpit and Trujillo, Mario F},
	doi = {10.1177/1468087419875843},
	issn = {1468-0874},
	journal = {International Journal of Engine Research},
	month = {jan},
	number = {1},
	pages = {55--72},
	title = {{The effect of nozzle internal flow on spray atomization}},
	volume = {21},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1177/1468087419875843}}

@article{Rupp2020,
	author = {Rupp, Matthias and Rieke, Christian and Handschuh, Nils and Kuperjans, Isabel},
	doi = {10.1016/j.trd.2020.102293},
	journal = {Transportation Research Part D: Transport and Environment},
	title = {{Economic and ecological optimization of electric bus charging considering variable electricity prices and CO2eq intensities}},
	volume = {81},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.trd.2020.102293}}

@article{Qiu2015,
	author = {Qiu, Lu and Reitz, Rolf D.},
	doi = {10.1016/j.ijmultiphaseflow.2015.01.011},
	journal = {International Journal of Multiphase Flow},
	pages = {24--38},
	title = {{An investigation of thermodynamic states during high-pressure fuel injection using equilibrium thermodynamics}},
	volume = {72},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2015.01.011}}

@article{Matheis2018,
	author = {Matheis, Jan and Hickel, Stefan},
	doi = {10.1016/j.ijmultiphaseflow.2017.11.001},
	journal = {International Journal of Multiphase Flow},
	pages = {294 --311},
	title = {{Multi-component vapor-liquid equilibrium model for LES of high-pressure fuel injection and application to ECN Spray A}},
	volume = {99},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2017.11.001}}

@phdthesis{Blanco2016,
	author = {Blanco, A.P.},
	school = {Polytechnic University of Valencia},
	title = {{Implementation and Development of an Eulerian Spray Model for CFD Simulations of Diesel Sprays}},
	year = {2016}}

@inproceedings{Shashank2011,
	author = {Shashank and Knudsen, E. and Pitsch, H.},
	booktitle = {Annual Research Briefs, Center for Turbulence Research},
	title = {Spray evaporation model sensitivities},
	year = {2011}}

@article{Anez2019,
	author = {Anez, J. and Ahmed, A. and Hecht, N. and Duret, B. and Reveillon, J. and Demoulin, F.X.},
	doi = {10.1016/j.ijmultiphaseflow.2018.10.009},
	journal = {International Journal of Multiphase Flow},
	pages = {325--342},
	title = {{Eulerian--Lagrangian spray atomization model coupled with interface capturing method for diesel injectors}},
	volume = {113},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2018.10.009}}

@article{Desantes2020,
	author = {Desantes, J.M. and Garc{\'\i}a-Oliver, J.M. and Pastor, J.M. and Olmeda, I. and Pandal, A. and Naud, B.},
	doi = {10.1016/j.ijmultiphaseflow.2020.103272},
	journal = {International Journal of Multiphase Flow},
	pages = {103272},
	title = {{LES Eulerian diffuse-interface modeling of fuel dense sprays near- and far-field}},
	volume = {127},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2020.103272}}

@article{Garcia2013,
	author = {Garcia-Oliver, Jose M. and Pastor, Jose M. and Pandal, Adrian and Trask, N. and Baldwin, E. and Schmidt, David P.},
	doi = {10.1615/AtomizSpr.2013007198},
	journal = {Atomization and Sprays},
	number = {1},
	pages = {71--95},
	title = {{Diesel Spray CFD Simulations based on the $\Sigma$-Y Eulerian Atomization}},
	volume = {23},
	year = {2013},
	Bdsk-Url-1 = {https://doi.org/10.1615/AtomizSpr.2013007198}}

@book{Crowe2012,
	author = {Crowe, C. T. and Schwarzkopf, J. D. and Sommerfeld, M. and Tsuji, Y.},
	publisher = {Taylor \& Francis Group, LLC},
	title = {{Mulitphase Flows with Droplets and Particles}},
	year = {2012}}

@book{Wallis1969,
	author = {Wallis, G. B.},
	publisher = {McGraw-Hill, New York},
	title = {{One-Dimensional Two-Phase Flow}},
	year = {1969}}

@article{Pitsch1995,
	author = {Pitsch, H. and Wan, Y. and Peters, N.},
	doi = {10.4271/952357},
	journal = {SAE Technical Paper 952357},
	title = {{Numerical Investigation of Soot Formation and Oxidation under Diesel Engine Conditions}},
	year = {1995},
	Bdsk-Url-1 = {https://doi.org/10.4271/952357}}

@article{Pitsch1996,
	author = {Pitsch, H. and Barths, H. and Peters, N.},
	doi = {10.4271/962057},
	journal = {SAE Technical Paper 962057},
	title = {{Three-Dimensional Modeling of NOx and Soot Formation in DI-Diesel Engines Using Detailed Chemistry Based on the Interactive Flamelet Approach}},
	year = {1996},
	Bdsk-Url-1 = {https://doi.org/10.4271/962057}}

@article{Barths1999,
	author = {Barths, H. and Pitsch, H. and Peters, N.},
	doi = {10.2516/ogst:1999020},
	journal = {Oil {\&} Gas Science and Technology -- Revue d'IFP Energies nouvelles},
	number = {2},
	pages = {233--244},
	title = {{3D Simulation of DI Diesel Combustion and Pollutant Formation Using a Two-Component Reference Fuel}},
	volume = {54},
	year = {1999},
	Bdsk-Url-1 = {https://doi.org/10.2516/ogst:1999020}}

@article{Barths2000,
	author = {Barths, H. and Hasse, C. and Bikas, G. and Peters, N.},
	doi = {10.1016/S0082-0784(00)80326-4},
	journal = {Proceedings of the Combustion Institute},
	number = {1},
	pages = {1161--1168},
	title = {{Simulation of Combustion in Direct Injection Diesel Engines using a Eulerian Particle Flamelet Model}},
	volume = {28},
	year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0082-0784(00)80326-4}}

@inproceedings{Pitsch1998,
	author = {Pitsch, H. and Chen, M. and Peters, N.},
	booktitle = {27th International Symposium on Combustion, The Combustion Institute},
	pages = {1057--1064},
	title = {{Unsteady Flamelet Modeling of Turbulent Hydrogen/Air Diffusion Flames}},
	volume = {27},
	year = {1998}}

@article{Derrico2014,
	author = {G. D'Errico and T. Lucchini and F. Contino and M. Jangi and X.-S. Bai},
	doi = {10.1080/13647830.2013.860238},
	journal = {Combustion Theory and Modelling},
	number = {1},
	pages = {65--88},
	publisher = {Taylor & Francis},
	title = {Comparison of well-mixed and multiple representative interactive flamelet approaches for diesel spray combustion modelling},
	volume = {18},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1080/13647830.2013.860238}}

@article{Ottenwaelder2017,
	author = {Ottenw\"alder, T. and Pischinger, S.},
	doi = {10.4271/2017-01-2332},
	journal = {SAE Technical Paper 2017-01-2332},
	title = {{Effects of Biofuels on the Mixture Formation and Ignition Process in Diesel-Like Jets}},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.4271/2017-01-2332}}

@article{Cai2015,
	author = {Cai, Liming and Pitsch, Heinz},
	doi = {10.1016/j.combustflame.2014.11.018},
	journal = {Combustion and Flame},
	number = {5},
	pages = {1623--1637},
	title = {{Optimized chemical mechanism for combustion of gasoline surrogate fuels}},
	volume = {162},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2014.11.018}}

@article{Frassoldati2015,
	author = {Frassoldati, Alessio and D'Errico, Gianluca and Lucchini, Tommaso and Stagni, Alessandro and Cuoci, Alberto and Faravelli, Tiziano and Onorati, Angelo and Ranzi, Eliseo},
	doi = {10.1016/j.combustflame.2015.07.039},
	journal = {Combustion and Flame},
	number = {10},
	pages = {3991--4007},
	title = {{Reduced kinetic mechanisms of diesel fuel surrogate for engine CFD simulations}},
	volume = {162},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2015.07.039}}

@article{Yao2017,
	author = {Yao, Tong and Pei, Yuanjiang and Zhong, Bei-Jing and Som, Sibendu and Lu, Tianfeng and Luo, Kai Hong},
	doi = {10.1016/j.fuel.2016.11.083},
	journal = {Fuel},
	pages = {339--349},
	title = {{A compact skeletal mechanism for n-dodecane with optimized semi-global low-temperature chemistry for diesel engine simulations}},
	volume = {191},
	year = {2017},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2016.11.083}}

@inproceedings{Cai2015a,
	address = {Avignon, France},
	author = {Cai, L. and Kr\"oger, L. and Pitsch, H.},
	booktitle = {Fifteenth International Conference on Numerical Combustion},
	day = {19th--22nd},
	month = {April},
	title = {{Reduced and Optimized Mechanism for N-Dodecane Oxidation}},
	year = {2015}}

@article{Cai2015b,
	author = {Cai, Liming and Uygun, Yasar and Togb\'e, Casimir and Pitsch, Heinz and Olivier, Herbert and Dagaut, Philippe and Sarathy, S. Mani},
	doi = {10.1016/j.proci.2014.05.088},
	journal = {Proceedings of the Combustion Institute},
	number = {1},
	pages = {419--427},
	title = {{An experimental and modeling study of n-octanol combustion}},
	volume = {35},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.proci.2014.05.088}}

@article{Pickett2004,
	author = {Pickett, Lyle M. and Siebers, Dennis L.},
	doi = {10.1016/j.combustflame.2004.04.006},
	journal = {Combustion and Flame},
	number = {1},
	pages = {114--135},
	title = {{Soot in diesel fuel jets: effects of ambient temperature, ambient density, and injection pressure}},
	volume = {138},
	year = {2004},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2004.04.006}}

@article{Cai2014,
	author = {Cai, Liming and Alena Sudholt and Lee, Dong Joon and Egolfopoulos, Fokion N. and Pitsch, Heinz and Westbrook, Charles K. and Sarathy, S. Mani},
	doi = {10.1016/j.combustflame.2013.10.003},
	journal = {Combustion and Flame},
	note = {Special Issue on Alternative Fuels},
	number = {3},
	pages = {798--809},
	title = {{Chemical kinetic study of a novel lignocellulosic biofuel: Di-n-butyl ether oxidation in a laminar flow reactor and flames}},
	volume = {161},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2013.10.003}}

@article{Cai2020,
	author = {Cai, Liming and Jacobs, Sascha and Langer, Raymond and {vom Lehn}, Florian and Heufer, Karl Alexander and Pitsch, Heinz},
	doi = {10.1016/j.fuel.2019.116711},
	journal = {Fuel},
	pages = {116711},
	title = {{Auto-ignition of oxymethylene ethers (OMEn, n = 2--4) as promising synthetic e-fuels from renewable electricity: shock tube experiments and automatic mechanism generation}},
	volume = {264},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.fuel.2019.116711}}

@article{Jacobs2019,
	author = {Jacobs, S. and D{\"o}ntgen, M. and Alquaity, A.B.S. and Kopp, W.A. and Kr{\"o}ger, L.C. and Burke, U. and Pitsch, H. and Leonhard, K. and Curran, H.J. and Heufer, K.A.},
	doi = {10.1016/j.combustflame.2018.12.026},
	journal = {Combustion and Flame},
	pages = {522--533},
	title = {{Detailed kinetic modeling of dimethoxymethane. Part II: Experimental and theoretical study of the kinetics and reaction mechanism}},
	volume = {205},
	year = {2019},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2018.12.026}}

@article{Deshmukh2022,
	author = {Deshmukh, A. Y. and Grenga, T. and Davidovic, M. and Schumacher, L. and Palmer, J. and Reddemann, M. A. and Kneer, R. and Pitsch, H.},
	date-modified = {2023-03-21 08:17:24 +0100},
	doi = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103872},
	journal = {Internation Journal of Multiphase Flows},
	pages = {103872},
	title = {A Reduced-order Model for Multiphase Simulation of Transient Inert Sprays},
	volume = {147},
	year = {2022},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.ijmultiphaseflow.2021.103872}}

@article{Mueller2009,
	author = {Mueller, M.E. and Blanquart, G. and Pitsch, H.},
	doi = {10.1016/j.combustflame.2009.01.025},
	journal = {Combustion and Flame},
	number = {6},
	pages = {1143--1155},
	title = {{Hybrid Method of Moments for modeling soot formation and growth}},
	volume = {156},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2009.01.025}}

@article{Raman2006,
	author = {Raman, Venkatramanan and Pitsch, Heinz and Fox, Rodney O.},
	doi = {10.1080/13647830500460474},
	journal = {Combustion Theory and Modelling},
	number = {3},
	pages = {439--458},
	publisher = {Taylor & Francis},
	title = {{Eulerian transported probability density function sub-filter model for large-eddy simulations of turbulent combustion}},
	volume = {10},
	year = {2006},
	Bdsk-Url-1 = {https://doi.org/10.1080/13647830500460474}}

@article{Frenklach1991,
	author = {Frenklach , Michael and Wang, Hai},
	doi = {10.1016/S0082-0784(06)80426-1},
	journal = {Symposium (International) on Combustion},
	note = {Twenty-Third Symposium (International) on Combustion},
	number = {1},
	pages = {1559--1566},
	title = {{Detailed modeling of soot particle nucleation and growth}},
	volume = {23},
	year = {1991},
	Bdsk-Url-1 = {https://doi.org/10.1016/S0082-0784(06)80426-1}}

@article{Frenklach2002,
	author = {Frenklach, Michael},
	doi = {10.1039/B110045A},
	issue = {11},
	journal = {Phys. Chem. Chem. Phys.},
	pages = {2028--2037},
	publisher = {The Royal Society of Chemistry},
	title = {{Reaction mechanism of soot formation in flames}},
	volume = {4},
	year = {2002},
	Bdsk-Url-1 = {https://doi.org/10.1039/B110045A}}

@article{Blanquart2009,
	author = {Blanquart, G. and Pitsch, H.},
	doi = {10.1016/j.combustflame.2009.04.010},
	issn = {0010-2180},
	journal = {Combustion and Flame},
	number = {8},
	pages = {1614--1626},
	title = {{Analyzing the effects of temperature on soot formation with a joint volume-surface-hydrogen model}},
	volume = {156},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2009.04.010}}

@article{Hubbard1978,
	author = {Hubbard, G. L. and Tien, C. L.},
	doi = {10.1115/1.3450788},
	journal = {Journal of Heat Transfer},
	month = {05},
	number = {2},
	pages = {235--239},
	title = {{Infrared Mean Absorption Coefficients of Luminous Flames and Smoke}},
	volume = {100},
	year = {1978},
	Bdsk-Url-1 = {https://doi.org/10.1115/1.3450788}}

@article{Grosshandler1993,
	author = {Grosshandler, William L.},
	journal = {NIST technical note 1402},
	month = {04},
	title = {{RADCAL: A Narrow-Band Model for Radiation Calculations in a Combustion Environment}},
	year = {1993}}

@article{Pitsch2000,
	author = {Pitsch, H. and Riesmeier, E. and Peters, N.},
	doi = {10.1080/00102200008947342},
	journal = {Combustion Science and Technology},
	number = {1},
	pages = {389--406},
	publisher = {Taylor & Francis},
	title = {{Unsteady Flamelet Modeling of Soot Formation in Turbulent Diffusion Flames}},
	volume = {158},
	year = {2000},
	Bdsk-Url-1 = {https://doi.org/10.1080/00102200008947342}}

@article{Cai2016,
	author = {Cai, Liming and Pitsch, Heinz and Mohamed, Samah Y. and Raman, Venkat and Bugler, John and Curran, Henry and Sarathy, S. Mani},
	doi = {10.1016/j.combustflame.2016.04.022},
	journal = {Combustion and Flame},
	pages = {468--482},
	title = {{Optimized reaction mechanism rate rules for ignition of normal alkanes}},
	volume = {173},
	year = {2016},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2016.04.022}}

@article{Blanquart2009a,
	author = {Blanquart, G. and Pepiot-Desjardins P. and Pitsch, H.},
	doi = {10.1016/j.combustflame.2008.12.007},
	journal = {Combustion and Flame},
	number = {3},
	pages = {588--607},
	title = {{Chemical mechanism for high temperature combustion of engine relevant fuels with emphasis on soot precursors}},
	volume = {156},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.combustflame.2008.12.007}}

@article{Albrecht2007,
	author = {Albrecht, A. and Grondin, O. and Berr, F. Le and Solliec, G. Le},
	doi = {10.2516/ogst:2007039},
	journal = {Oil {\&} Gas Science and Technology -- Revue d'IFP Energies nouvelles},
	number = {4},
	pages = {437--456},
	title = {{Towards a Stronger Simulation Support for Engine Control Design: a Methodological Point of View}},
	volume = {62},
	year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.2516/ogst:2007039}}

@article{Bengtsson2007,
	author = {Bengtsson, J. and Strandh, P. and Johansson, R. and Tunest\r{a}l, P. and Johansson, B.},
	doi = {10.1080/00207170701484869},
	journal = {International Journal of Control},
	number = {11},
	pages = {1814-1847},
	publisher = {Taylor & Francis},
	title = {{Hybrid modelling of homogeneous charge compression ignition (HCCI) engine dynamics---a survey}},
	volume = {80},
	year = {2007},
	Bdsk-Url-1 = {https://doi.org/10.1080/00207170701484869}}

@article{Hillion2009,
	author = {Hillion, M. and Buhlbuck, H. and Chauvin, J. and Petit, N.},
	doi = {10.4271/2009-01-0367},
	journal = {SAE Technical Paper 2009-01-0367},
	title = {{Combustion Control of Diesel Engines Using Injection Timing}},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.4271/2009-01-0367}}

@inproceedings{Korkmaz2018,
	address = {Aachen, Germany},
	author = {Korkmaz, Metin and Golc, Dominik and Jochim, Bernhard and Beeckmann, Joachim and Heinz Pitsch},
	booktitle = {Symposium for Combustion Control},
	date = {27th-28th},
	month = {June},
	title = {{Development of a Fully Flexible Injection Strategy for Model-Based Combustion Control of PCCI Diesel Engine}},
	year = {2018}}

@article{Korkmaz2018a,
	author = {Korkmaz, Metin and Zweigel, Ren{\'e} and Jochim, Bernhard and Beeckmann, Joachim and Abel, Dirk and Heinz Pitsch},
	doi = {10.1177/1468087417730485},
	journal = {International Journal of Engine Research},
	number = {2},
	pages = {230--240},
	title = {{Triple-injection strategy for modelbased control of premixed charge compression ignition diesel engine combustion}},
	volume = {19},
	year = {2018},
	Bdsk-Url-1 = {https://doi.org/10.1177/1468087417730485}}

@inproceedings{Ritter2017,
	address = {Berlin, Germany},
	author = {Ritter, Dennis and Korkmaz, Metin and Pitsch, Heinz and Abel, Dirk and Albin, Thivaharan},
	booktitle = {AUTOREG 2017 -- Automatisiertes Fahren und vernetzte Mobilit{\"a}t},
	date = {5th-6th},
	month = {June},
	publisher = {VDI/VDE Fachtagung},
	title = {{Model-based Control of CNG-Diesel Dual-Fuel Engines}},
	volume = {8},
	year = {2017}}

@article{Arregle2003a,
	author = {Arr\'{e}gle, J. and L\'{o}pez, J.J. and Garc\'{i}a, J.M. and Fenollosa, C.},
	doi = {10.1016/S1359-4311(03)00079-6},
	journal = {Applied Thermal Engineering},
	number = {11},
	pages = {1301--1317},
	title = {{Development of a zero-dimensional Diesel combustion model. Part 1: Analysis of the quasi-steady diffusion combustion phase}},
	volume = {23},
	year = {2003},
	Bdsk-Url-1 = {https://doi.org/10.1016/S1359-4311(03)00079-6}}

@article{Arregle2003b,
	author = {Arr\'{e}gle, J. and L\'{o}pez, J.J. and Garc\'{i}a, J.M. and Fenollosa, C.},
	doi = {10.1016/S1359-4311(03)00080-2},
	journal = {Applied Thermal Engineering},
	number = {11},
	pages = {1319--1331},
	title = {{Development of a zero-dimensional Diesel combustion model: Part 2: Analysis of the transient initial and final diffusion combustion phases}},
	volume = {23},
	year = {2003},
	Bdsk-Url-1 = {https://doi.org/10.1016/S1359-4311(03)00080-2}}

@article{Whitehouse1962,
	author = {Whitehouse, N. D. and Stotter, A. and Goudie, G. O. and Prentice, B. W.},
	doi = {10.1243/PIME\_PROC\_1962\_176\_022\_02},
	journal = {Proceedings of the Institution of Mechanical Engineers},
	number = {1},
	pages = {195--217},
	title = {{Method of Predicting Some Aspects of Performance of a Diesel Engine Using a Digital Computer}},
	volume = {176},
	year = {1962},
	Bdsk-Url-1 = {https://doi.org/10.1243/PIME%5C_PROC%5C_1962%5C_176%5C_022%5C_02}}

@article{Garcia2020,
	author = {Garcia-Oliver, J. and Novella, R. and Pastor, J. and Pachano, L.},
	doi = {10.4271/2020-01-0661},
	journal = {SAE International Journal of Advances and Current Practices in Mobility},
	number = {4},
	pages = {1974--1985},
	title = {{A Quasi-1D Model for the Description of ECN Spray a Combustion Process}},
	volume = {2},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.4271/2020-01-0661}}

@article{Ma2014,
	author = {Ma, Guanqin and Tauzia, Xavier and Maiboom, Alain},
	doi = {10.1177/0954407013518036},
	journal = {Proceedings of the Institution of Mechanical Engineers, Part D: Journal of Automobile Engineering},
	number = {4},
	pages = {457--476},
	title = {{One-dimensional combustion model with detailed chemistry for transient diesel sprays}},
	volume = {228},
	year = {2014},
	Bdsk-Url-1 = {https://doi.org/10.1177/0954407013518036}}

@article{Felsch2009,
	author = {Felsch, C. and Hoffmann, K. and Vanegas, A. and Drews, P. and Barths, H. and Abel, D. and Peters, N.},
	doi = {10.1243/14680874JER04509},
	journal = {International Journal of Engine Research},
	number = {6},
	pages = {359-387},
	title = {{Combustion model reduction for diesel engine control design}},
	volume = {10},
	year = {2009},
	Bdsk-Url-1 = {https://doi.org/10.1243/14680874JER04509}}

@inproceedings{Zweigel2015,
	author = {Zweigel, R. and Thelen, F. and Abel, D. and Albin, T.},
	booktitle = {2015 European Control Conference (ECC)},
	doi = {10.1109/ECC.2015.7331021},
	pages = {3168--3173},
	title = {{Iterative learning approach for diesel combustion control using injection rate shaping}},
	year = {2015},
	Bdsk-Url-1 = {https://doi.org/10.1109/ECC.2015.7331021}}

@article{Launder1974,
	author = {Launder, B.E. and Spalding, D.B.},
	doi = {10.1016/0045-7825(74)90029-2},
	journal = {Computer Methods in Applied Mechanics and Engineering},
	number = {2},
	pages = {269--289},
	title = {{The numerical computation of turbulent flows}},
	volume = {3},
	year = {1974},
	Bdsk-Url-1 = {https://doi.org/10.1016/0045-7825(74)90029-2}}

@article{Hubbard1975,
	author = {Hubbard, G. and Denny, V. and Mills, A.},
	doi = {10.1016/0017-9310(75)90217-3},
	journal = {International Journal of Heat and Mass Transfer},
	pages = {1003--1008},
	title = {{Droplet evaporation: Effects of transients and variable properties}},
	volume = {18},
	year = {1975},
	Bdsk-Url-1 = {https://doi.org/10.1016/0017-9310(75)90217-3}}

@article{Maes2020,
	author = {Maes, Noud and Skeen, Scott A. and Bardi, Michele and Fitzgerald, Russell P. and Malbec, Louis-Marie and Bruneaux, Gilles and Pickett, Lyle M. and Yasutomi, Koji and Martin, Glen},
	doi = {10.1016/j.applthermaleng.2020.115136},
	journal = {Applied Thermal Engineering},
	pages = {115136},
	title = {{Spray penetration, combustion, and soot formation characteristics of the ECN Spray C and Spray D injectors in multiple combustion facilities}},
	volume = {172},
	year = {2020},
	Bdsk-Url-1 = {https://doi.org/10.1016/j.applthermaleng.2020.115136}}

